Preliminaries paper: Byzantine Tolerant Strong Auditable Atomic Register

An auditable register extends the classical register with an audit operation that returns information on the read operations performed on the register. In this paper, we study Byzantine resilient auditable register implementations in an asynchronous message-passing system. Existing solutions implement the auditable register on top of at least 4f+1 servers, where at most $f$ can be Byzantine. We show that 4f+1 servers are necessary to implement auditability without communication between servers, or implement does not implement strong auditability when relaxing the constraint on the servers' communication, letting them interact with each other. In this setting, it exists a solution using 3f+1 servers to implement a simple auditable atomic register. In this work, we implement strong auditable register using 3f+1 servers with server to server communication, this result reinforced that with communication between servers, auditability (event strong auditability) does not come with an additional cost in terms of the number of servers.

==> Legacy/algorithmsLegacy/asynchronousCase/auditClientAsyncUnbound.tex <==
\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]

\Statex Initialization
\Statex $ ts \gets 0$ \label{line:async:unbound:initTs}
\Statex $ b_i \gets \perp\, \forall i  \in [1,n]$
% \Statex $\CR \gets \emptyset$
% \Statex $\concurrentReaderProof \gets \emptyset$
\Statex $ \writerAcks[i] \gets \perp,\, \forall i  \in [1,n]$

\Statex


\START[Write]($v$)\{
% \State $ CR \gets \perp$
\State{$ts \gets ts+1$} \label{line:async:unbound:incts}
\State{$[b_1,\ldots,b_n]\gets \generatesBlock(v) $} 
% \Comment{{\tiny $b_i$ is encrypted with the public key of $\ps{i}$} }

% \State \CR = \GetConcurrentReaders()
% \Statex{// Phase W1 Round 1}
% \START[for] $i \in [1,n]$ $send(\nextval,$ $ts,$ $b_i)$ to server $\ps{i}$

% \START[\texttt{broadcast{]$(\nextval,$ $ts,$ $[b_1,\ldots,b_n])$ to all servers
% \label{line:async:unbound:nextVal}
% \EndPhase
% \START[repeat]
% \State{ // Wait responses}
% \EndPhase
% \State \textbf{until} (receives $n-f$ $\nextvalack$ messages) \textcolor{red}{f+1? to check if the proof still works with this threshold}
% \label{line:async:unbound:nextValWait}

% \State $\CR,\concurrentReaderProof\gets \GetConcurrentReaders(ts)$
% \label{line:async:unbound:concurrentReaderSubProtocol}
% \Comment{The detection of concurrent reader assure the termination in the case of numerous concurrent write to the read operation}
% \Statex // Phase W2 Round 2

\START[\texttt{broadcast}]$(\writets,ts,[b_1,\ldots,b_n])$ to all servers
\label{line:async:unbound:writeTs}
\EndPhase
% \START[repeat]
% \Statex{ // Wait responses}
% \EndPhase
% \State \textbf{until} (receives $n-f$ $\writetsack$ messages from different servers)
\State{\textbf{wait until} $|\{x:\writerAcks[x]= ts\}|\geq n-f$}
\label{line:async:unbound:writeTsWaitAck}

\State{\textbf{return}}
\EndPhase
\Statex \}
\Statex

\START[upon \texttt{receive}] ($\writetsack,t$) from server $\ps{i}$
\START[if] ($ts=t$) \,\{ $\writerAcks[i]\gets t$\}
\EndPhase
\EndPhase

\Statex
% \START[$\GetConcurrentReaders(ts)$]
% \Statex $ \readers[i] \gets \emptyset\, \forall i  \in [1,n]$
% % \START[for] $i \in [1,n]$ $send(\getReaders,ts)$ to server $\ps{i}$
% \START[\texttt{broadcast}] $(\getReaders,ts)$ to all servers
% \label{line:async:unbound:broadcastConcurrentReader}
% \EndPhase
% \START[repeat]
% \START[on \texttt{receive}] ($\sendReaders,\READERS_{i},ts$) from server $\ps{i}$
% \State $\readers[i]\gets \READERS_{i}$
% \EndPhase
% \EndPhase {\textbf{until} (n-f) responses from different servers}
% \label{line:async:unbound:waitConcurrentReader}
% \State{$\CR=\{r:|\{r\in\readers[i], \forall i \in [1,n]\}|\geq f+1\}$}
% \label{line:async:unbound:conditionAddConcurrentReader}
% \START[for each] $r\in\CR$
% \State $\concurrentReaderProof \gets \concurrentReaderProof \cup \sigma_{\pw}(r,ts)$
% \EndPhase
% \State{\textbf{return} $\CR,\concurrentReaderProof$}
% \label{line:async:unbound:returnConcurrentReader}

% \EndPhase

\START[Audit()]\{
\label{line:async:unbound:auditStart}
\Statex $\collectedLog[i] \gets \emptyset, \forall i \in [1,n] $
\START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\AuditReq)$ to server $\ps{i}$
\label{line:async:unbound:auditRequest}
\EndPhase
\State \textbf{wait until} $ |\{i:\collectedLog[i]\not=\emptyset\}|\geq n-f$
\label{line:async:unbound:waitAuditResponse}
\START[for] \textbf{all}$(\pr,ts,\nSeq)\in \bigcup_{i\in[1,n]}\collectedLog[i]$ %\textbf{do}
% \START[for] \textbf{all} $(\pr,v,wsn,rsn)$ with wsn the greatest sequence number
\START[for] $1\leq k\leq n$  \textbf{if} $(\pr,ts,\nSeq)_{\sigma_{\pr}} \in \collectedLog[k]$  $\land(\pr,ts,\nSeq)_{\sigma_{\pr}}\not \in E_A$
\State\textbf{then} $E_A\gets E_A\cup (\pr,ts,\nSeq)_{\sigma_{\pr}}$
\EndPhase
% \textbf{then} $\mathcal{E}_{\pr,ts,\nSeq}\gets\mathcal{E}_{\pr,ts,\nSeq}\cup\{k\} $
% \State{\textbf{if} $|\mathcal{E}_{\pr,ts,\nSeq}|\geq =t$ \textbf{then} $E_A\gets E_A\cup (\pr,ts,\nSeq)_{\sigma_{\pr}} $}
\label{line:async:unbound:conditionReportAudit}
% \EndPhase
\EndPhase
\State{\textbf{return} $E_A$} 
\label{line:async:unbound:auditEnd}
% \Comment{For the accountability use sign message}

\EndPhase
\Statex \}

\START[upon \texttt{receive}] ($\AuditResp, \Logi$) from server $\ps{i}$
\State \textbf{if} $\Logi=\emptyset$ \textbf{then} \{ $\collectedLog[i]\gets \perp$ \}
\State \textbf{else} $\collectedLog[i]\gets \Logi$
\EndPhase

\end{algorithmic}
}
    \caption{Pseudo-code of the write and audit operations at writer $\pw$.}
    \label{alg:async:unbound:AtomicRegisterClientWrite}
\end{figure}







\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Definitions:}
% \Statex $\ValidBlock( \langle ts\rangle) \triangleq \{v|\exists \{b\}\in Values[ts], \GetBlock(\{b\})=v\}\land valid(v)$ 
\Statex $\ValidBlock(ts) \triangleq  {\sf \GetValue} (\collectedValues)=(v,ts)$ 
% \Statex $\notOld(ts) \triangleq |\{i:max(\collectedTs[i])\leq ts\}|\geq 2f+1$
\Statex \textcolor{black}{ $\notOld( ts) \triangleq |\{i:min(\collectedTs[i])\leq ts\}|\geq 2f+1$ }
\Statex


\Statex \textbf{Initialization :}
\Statex $\nSeq \gets 0$
\Statex $\collectedValues[i] \gets (\perp,\perp), \forall i \in [1,n] $
\Statex $\collectedTs[i] \gets \emptyset, \forall i \in [1,n] $
\Statex $\smallestTimestamp \gets \perp$
\Statex
\START[Read()]\{
\State{$\nSeq \gets \nSeq+1$}
\State $\collectedValues[i] \gets (\perp,\perp), \forall i \in [1,n] $
\State $\collectedTs[i] \gets \emptyset, \forall i \in [1,n] $
% \State $\fwd[i] \gets \perp, \forall i \in [1,n]$
\State $\smallestTimestamp \gets \perp$

% \START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\getts,\nSeq)$ to server $\ps{i}$
% \EndPhase
\START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\getts,\nSeq)$ to server $\ps{i}$
\label{line:async:unbound:sendGetTs}

\EndPhase
\State \textbf{wait until}
$(|\{ts\in\collectedTs:ts=\smallestTimestamp\}|\geq f+1)$
\label{line:async:unbound:conditionGetBlock}

% \START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\GetBlocks,(\pr,\smallestTimestamp,\nSeq)_{\sigma(\pr)})$ \Statex 
% \hfill to server $\ps{i}$
% \EndPhase
\START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\GetBlocks,(\pr,\smallestTimestamp,\nSeq)_{\sigma_{\pr}})$  to server $\ps{i}$
\label{line:async:unbound:sendGetBlocks}
\EndPhase

\State \textbf{wait until}
$(\ValidBlock(ts)\land\notOld(ts))$
\label{line:async:unbound:conditionread}

\label{line:async:unbound:endReadMessage}
\State \textbf{return}  $\GetValue(\collectedValues)$
\label{line:async:unbound:readReturn}

\EndPhase
\Statex
\Statex

\START[upon \texttt{receive}]{ (\TS,ts,num) from server $\ps{i}$}
\START[if] ($num=\nSeq$)
    \State $\collectedTs[i]\gets \collectedTs[i]\cup ts$
    \label{line:async:unbound:tsRepColectTs}
    \START[if] $(|x:\collectedTs[x]\not=\perp\}|\geq n-f$
    \State\textcolor{black}{ $\smallestTimestamp \gets min(\{ts\in \collectedTs$ $|$ $\notOld(ts)\})$}
    \label{line:async:unbound:notOld}
    % \START[for] { $i \in [1,n]$
    % \texttt{\textbf{send}} $(\GetValUnbound,\smallestTimestamp$, \Statex \hfill $\nSeq)$ to server $\ps{i}$}
    % \EndPhase
    \START[for] $i \in  [1,n]$ \texttt{\textbf{send}} $(\GetValUnbound,\smallestTimestamp,\nSeq)$  to server $\ps{i}$
    \label{line:async:unbound:sendGetVal}
    \EndPhase
    
    % \State \texttt{\textbf{send}} $(\GetValUnbound,\smallestTimestamp,\nSeq)$ to all servers
    % \label{line:async:unbound:sendGetVal}
    \EndPhase
    \EndPhase
\EndPhase

\Statex

\START[upon \texttt{receive}] ($\SendValUnbound,ts,num$) from server $\ps{i}$
\START[if] ($num=\nSeq$)
\{$\collectedTs[i]\gets \collectedTs[i]\cup ts$\}
\label{line:async:unbound:valRepColectTs}
    \EndPhase
\EndPhase
\Statex

\START[upon \texttt{receive}]{ ($\SendBlock,b_{i},ts,num$) from server $\ps{i}$}
\START[if] ($num=\nSeq$)
    % \State $\fwd[i]\gets (b_{i},ts)$
    \State $\collectedValues[i]\gets (b_i,ts)$
    \label{line:async:unbound:ColectBlock}
    \EndPhase
\EndPhase



% \START[Read()]\{
% \Statex $\collectedTs[i] \gets \perp, \forall i \in [1,n] $
% \Statex $\collectedValues[i] \gets \emptyset, \forall i \in [1,n] $
% % \Statex $\forall i,\, \fwd[i] \gets \emptyset$
% \Statex $\smallestTimestamp \gets \perp$
% \Statex $\writtenBackVal \gets \langle \perp,\perp\rangle$
% % \Statex $phase \gets \perp$
% % \Statex $wb2cnt \gets 0$

% \Statex

% \Statex // Phase R1
% \START[for] $i \in  [1,n]$ $send(\getts)$ to server $\ps{i}$
% \label{line:async:unbound:sendGetTs}
% \EndPhase
% \START[repeat]
% \State // Wait responses

% \START[upon \texttt{receive}]{ (\TS,$\ps{i}$,ts) from server $\ps{i}$}
% \State $\collectedTs[i]\gets ts$
% \EndPhase
% % \START[upon \texttt{receive}]{ (\FWD,$\Vals_{i}$,ts) from server $\ps{i}$}
% % \State $\fwd[i]\gets \Vals_{i}$
% % \State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
% % \EndPhase
% % \State{// Wait responses}
% \EndPhase
% \State \textbf{until} $(|x:\collectedTs[x]\not=\perp\}|\geq n-f$
% \label{line:async:unbound:endPhaseR1}
% \Statex

% \Statex // Phase R2
% % \State $\phase \gets R2$
% \State{ $\smallestTimestamp \gets min(\{ts\in \collectedTs$ $|$ $\notOld(ts)\land \isSigned(ts)\})$}
% % \Comment{There is no write operation that terminates for a timestamp $t'>\smallestTimestamp$.}
% \START[for] $i \in  [1,n]$ $send(\getval,\smallestTimestamp,\textcolor{red}{\signMessage{\pr,\smallestTimestamp}{\pr}})$ to server $\ps{i}$
% \EndPhase

% % \State{$\smallestTimestamp \gets min(\{ts|\notOld(ts)==true\})$}
% % \START[for] $i \in  [1,n]$ $send(\getval,\smallestTimestamp)$ to server $i$
% \START[repeat]
% \State // Wait responses

% % \START[if]{$|\{\ps{i}, \collectedValues[i].ts=ts\}|\geq f+1$}
% % \START[for] $i \in  [1,n]$ send($\wbackval$,ts,$\collectedTsShare)$ to server $\ps{i}$
% % \label{line:async:unbound:writeBack1}
% % \EndPhase
% % \EndPhase
% % \START[upon \texttt{receive}]{ ($\FWD,\Vals_{i},ts$) from server $\ps{i}$}
% % \State $\fwd[i]\gets \Vals_{i}$
% % \State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
% % \EndPhase

% \Statex
% \START[upon \texttt{receive}]{ (\TS,$\ps{i}$,ts) from server $\ps{i}$}
% % \START[if] {$\phase=R2\lor\phase=R1$}
% \State $\collectedTs[i]\gets ts$
% % \EndPhase
% % \START[if] {$\phase=R2$}
% \State{\tiny $\smallestTimestamp \gets min(\{ts\in \collectedTs$ $|$ $\notOld(ts)=true\langle \isSigned(ts,\pw)\})$} \label{line:async:unbound:notOld}
% % \Comment{There is no write operation that terminates for a timestamp $t'>\smallestTimestamp$.}
% \START[for] $i \in [1,n]$ $send(\GetValUnbound,\smallestTimestamp,\textcolor{red}{\signMessage{\pr,\smallestTimestamp}{\pr}})$ to server $\ps{i}$
% \label{line:async:unbound:sendGetVal}
% \EndPhase
% \EndPhase
% % \EndPhase

% \Statex

% \START[upon \texttt{receive}]($\SendValUnbound$,$\Vals_{i},\shareVal$) from server $\ps{i}$
% % \START[if] {$\phase=R2$}
% \State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
% % \State $\collectedValShare[s]\gets \shareVal$
% % \State $\collectedShares_r[s]\gets \collectedShares_r[s]\cup \Vals.share$
% \EndPhase
% % \EndPhase
% % \State // Wait responses
% \EndPhase
% \State \textbf{until}
% $(|ts:\collectedTs bis[i]=ts|\geq f+1)\land (\notOld(\langle ts\rangle))$
% \label{line:async:unbound:conditionread}
% % \Statex // Phase Wb2
% % \State{$phase \gets WB2$}
% \Statex // Phase R3
% \textcolor{red}{
% \START[for] $i \in  [1,n]$ $send(\GetSignature,ts,BLS)$ to server $\ps{i}$
% % \EndPhase
% }
% \label{line:async:unbound:BLSReadMessage}
% \START[repeat]
% \State // Wait responses
% \EndPhase
% \State \textbf{until} $ 2f+1 responses.$

% \Statex // Phase R4
% \textcolor{red}{
% \START[for] $i \in  [1,n]$ $send(\GetBlocks,ts,BLS)$ to server $\ps{i}$
% % \EndPhase
% }
% \label{line:async:unbound:BLSReadMessage}
% \START[repeat]
% \State // Wait responses
% \EndPhase
% \State \textbf{until} $ 2f+1 responses.$
% \State $\writtenBackVal \gets \GetValue( \langle ts,\collectedValues \rangle)$

% % \EndPhase
% % \START[repeat]
% % \State{// Wait responses}
% % \EndPhase
% % \State \textbf{until} (receives n-f $\wbacktsack$ messages)
% % \label{line:async:unbound:waitWritebackTsAck}
% \State \textbf{return} $\writtenBackVal$
% \label{line:async:unbound:readReturn}

% \EndPhase
% \Statex \}
% \Statex


\end{algorithmic}
}
\caption{Pseudo-code of the read operation at reader $\pr$.}
\label{alg:async:unbound:AtomicRegisterClientRead}
\end{figure}






% \begin{figure}[!htpb]
% {\footnotesize
% \begin{algorithmic}[1]

% \Statex

% \START[Audit()]\{
% \Statex $\collectedLog[i] \gets \emptyset, \forall i \in [1,n] $
% \START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\AuditReq)$ to server $\ps{i}$
% \label{line:async:unbound:auditRequest}
% \EndPhase
% \State \textbf{wait until} $ |\{i:\collectedLog[i]\not=\emptyset\}|\geq n-f$
% \label{line:async:unbound:waitAuditResponse}
% \START[for] \textbf{all}$(\pr,ts,\nSeq)\in \bigcup_{i\in[1,n]}\collectedLog[i]$ %\textbf{do}
% % \START[for] \textbf{all} $(\pr,v,wsn,rsn)$ with wsn the greatest sequence number
% \START[for] $1\leq k\leq n$  \textbf{if} $(\pr,ts,\nSeq)_{\sigma_{\pr}} \in \collectedLog[k]$
% \Statex \hfill $\land(\pr,ts,\nSeq)_{\sigma_{\pr}}\not \in E_A$
% \State\textbf{then} $E_A\gets E_A\cup (\pr,ts,\nSeq)_{\sigma_{\pr}}$
% \EndPhase
% % \textbf{then} $\mathcal{E}_{\pr,ts,\nSeq}\gets\mathcal{E}_{\pr,ts,\nSeq}\cup\{k\} $
% % \State{\textbf{if} $|\mathcal{E}_{\pr,ts,\nSeq}|\geq =t$ \textbf{then} $E_A\gets E_A\cup (\pr,ts,\nSeq)_{\sigma_{\pr}} $}
% \label{line:async:unbound:conditionReportAudit}
% % \EndPhase
% \EndPhase
% \State{\textbf{return} $E_A$} 
% % \Comment{For the accountability use sign message}

% \EndPhase
% \Statex \}

% \START[upon \texttt{receive}] ($\AuditResp, \Logi$) from server $\ps{i}$
% \State \textbf{if} $\Logi=\emptyset$ \textbf{then} \{ $\collectedLog[i]\gets \perp$ \}
% \State \textbf{else} $\collectedLog[i]\gets \Logi$
% \EndPhase

% \end{algorithmic}
% }
% \caption{Audit operation of \algAsyncRBSign\, solution.}
% \label{alg:async:unbound:AtomicRegisterClientAudit}
% \end{figure}






==> Legacy/algorithmsLegacy/asynchronousCase/auditClientSave.tex <==
\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]

\Statex Initialization
\Statex $ ts \gets 0$
\Statex $ b_i \gets \perp\, \forall i  \in [1,n]$
\Statex $\CR \gets \emptyset$

% \Statex $ sh_i \gets \perp\, \forall i  \in [1,n]$
\Statex

\START[Write]($v$)\{
% \State $ CR \gets \perp$
\State{$ts \gets ts+1$} \label{line:async:incts}
% \State{$[sh_{r_1},\ldots,sh_{r_n}]\gets \generateShares_r()$} \Comment{Used in WB1, to attest of f+1 received messages for ts}
% \State{$[sh_{wb_1},\ldots,sh_{wb_n}]\gets \generateShares_{wb}()$} \Comment{Used in WB2, to ensure that the WB1 has terminates}
\State{$[b_1,\ldots,b_n]\gets \generatesBlock(v) $} \Comment{{\tiny $b_i$ is encrypted with the public key of $\ps{i}$} }
% \State{$[sh_1,\ldots,sh_n]\gets \generateShares(v) $} \Comment{$\tau=2f+1$ blocks are required to read the value }

% \State \CR = \GetConcurrentReaders()
\Statex{// Phase W1 Round 1}
% \START[for] $i \in [1,n]$ $send(\nextval,$ $ts,$ $b_i)$ to server $\ps{i}$
\START[broadcast]$(\nextval,$ $ts,$ $b_i)$ to all servers
\textbf{}
\label{line:async:nextVal}
\EndPhase
\START[repeat]
\State{ // Wait responses}
\EndPhase
\State \textbf{until} (receives $n-f$ $\nextvalack$ messages)
\label{line:async:nextValWait}

\State $\CR\gets \GetConcurrentReaders(ts)$
\label{line:async:concurrentReaderSubProtocol}
\Comment{The detection of concurrent reader assure the termination in the case of numerous concurrent write to the read operation}
\Statex // Phase W2 Round 2
% \START[for] $i \in [1,n]$ $send(\writeval)$ to server $\ps{i}$
\START[broadcast]$(\writeval)$ to all servers
\label{line:async:writeVal}
\EndPhase
\START[repeat]
\State{ // Wait responses}
\EndPhase
\State \textbf{until} (receives $n-f$ $\writevalack$ messages \Statex
        \hfill  from different servers)
\label{line:async:writeValWaitAck}

\Statex // Phase W3 Round 3
% \State $wait \, \GetConcurrentReaders() \, terminates$
% \START[for] $i \in [1,n]$ $send(\writets,$ $ts,$ $\CR)$ to server $\ps{i}$
\START[broadcast]$(\writets,$ $ts,$ $\CR)$ to all servers
\label{line:async:writeTs}
\EndPhase
\START[repeat]
\Statex{ // Wait responses}
\EndPhase
\State \textbf{until} (receives $n-f$ $\writetsack$ messages from different servers)
\label{line:async:writeTsWaitAck}

\State{\textbf{return}}
\EndPhase
\Statex \}
\Statex

\START[$\GetConcurrentReaders(ts)$]
\Statex $ \readers[i] \gets \emptyset\, \forall i  \in [1,n]$
% \START[for] $i \in [1,n]$ $send(\getReaders,ts)$ to server $\ps{i}$
\START[broadcast] $(\getReaders,ts)$ to all servers
\label{line:async:broadcastConcurrentReader}
\EndPhase
\START[repeat]
\START[on receive] ($\sendReaders,\READERS_{i},ts$) from server $\ps{i}$
\State $\readers[i]\gets \READERS_{i}$
\EndPhase
\EndPhase {\textbf{until} (n-f) responses from different servers}
\label{line:async:waitConcurrentReader}
\State{$\CR=\{r:|\{r\in\readers[i], \forall i \in [1,n]\}|\geq f+1\}$}
\label{line:async:conditionAddConcurrentReader}
\State{\textbf{return} $\CR$}
\label{line:async:returnConcurrentReader}

\EndPhase
\end{algorithmic}
}
    \caption{Write operation of \algAsyncRBSign\, solution. Writer side. }
    \label{alg:async:AtomicRegisterClientWrite}
\end{figure}




\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Definitions:}
% \Statex $\valid( \langle ts\rangle) \triangleq |\{s:\langle ts;*\rangle \in Values[s] \}| =2f+1$
\Statex $\ValidBlock( \langle ts\rangle) \triangleq \{v|\exists \{b\}\in Values[ts], \GetBlock(\{b\})=v\}\land valid(v)$ \Comment{$\tau=2f+1$ blocks are required to get the value, and the validity can be attested by the reader}
% \Statex $\acceptable(\langle ts\rangle) \triangleq \exists s :\collectedTs[s]=ts\land \writingBack(ts)=false$
\Statex $\notOld(\langle ts\rangle ) \triangleq |\{\ps{i}:\collectedTs[i]\leq ts\}|\geq =2f+1$
\Comment{$ts$ is greater equal than at least $2f+1$ other timestamps collected.}

\Statex $\fwded( \langle ts\rangle) \triangleq |\{\ps{i}:fwd[i]=\langle ts\rangle \}|\geq 2f+1$
% \Statex $\GetShares(\langle ts \rangle) \triangleq \{ x|\exists s:\langle ts,x\rangle \in Values[s]\}$
\Statex



\START[Read()]\{
\Statex $\collectedValues[i] \gets \emptyset, \forall i \in [1,n] $
\Statex $\collectedTs[i] \gets \perp, \forall i \in [1,n] $
\Statex $\collectedTsShare[i] \gets \perp, \forall i \in [1,n]$
% \Statex $\forall i,\, \fwd[i] \gets \emptyset$
% \Statex $\forall ts,\, \writingBack[ts] = false $
\Statex $\smallestTimestamp \gets \perp$
\Statex $\writtenBackVal \gets \langle \perp,\perp\rangle$
% \Statex $phase \gets \perp$
% \Statex $wb2cnt \gets 0$

\Statex

\Statex // Phase R1
\START[for] $i \in  [1,n]$ $send(\getts)$ to server $\ps{i}$
\label{line:async:sendGetTs}
\EndPhase
\START[repeat]
\START[upon receive]{ (\TS,$\ps{i}$,ts) from server $\ps{i}$}
\State $\collectedTs[i]\gets ts$
\EndPhase
\START[upon receive]{ (\FWD,$\ps{i}$,$\RVal_{i}$,$\Vals_{i}$,ts) from server $\ps{i}$}
\State $\fwd[i]\gets \RVal_{i}$
\State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
\EndPhase
% \State{// Wait responses}
\EndPhase
\State \textbf{until} $(|x:\collectedTs[x]\not=\perp\}|\geq n-f$
\label{line:async:endPhaseR1}
\Statex

\Statex // Phase R2/WB1 
\State $\phase \gets R2$
\State{ $\smallestTimestamp \gets min(\{ts\in \collectedTs$ $|$ $\notOld(ts)=true\})$}
% \Comment{There is no write operation that terminates for a timestamp $t'>\smallestTimestamp$.}
\START[for] $i \in  [1,n]$ $send(\getval,\smallestTimestamp)$ to server $\ps{i}$
\EndPhase

% \State{$\smallestTimestamp \gets min(\{ts|\notOld(ts)==true\})$}
% \START[for] $i \in  [1,n]$ $send(\getval,\smallestTimestamp)$ to server $i$
\START[repeat]

\START[if]{$|\{\ps{i}, \collectedValues[i].ts=ts\}|\geq f+1$}
\START[for] $i \in  [1,n]$ send($\wbackval$,ts,$\collectedTsShare)$ to server $\ps{i}$
\label{line:async:writeBack1}
\EndPhase
\EndPhase
% \State // Wait responses
\EndPhase
\State \textbf{until}
$\ValidBlock( \langle ts\rangle)\land (\notOld(\langle ts\rangle)\lor \fwded(\langle ts\rangle))$
\label{line:async:conditionread}
\Statex // Phase Wb2
\State $\writtenBackVal \gets \GetBlock( \langle ts,\collectedValues \rangle)$
\START[for] $i \in  [1,n]$ $send(\wbackts,ts,\collectedTsShare)$ to server $\ps{i}$
\label{line:async:writeBack2}
\EndPhase
\START[repeat]
\State{// Wait responses}
\EndPhase
\State \textbf{until} (receives n-f $\wbacktsack$ messages)
\label{line:async:waitWritebackTsAck}
\State \textbf{return} $\writtenBackVal$
\label{line:async:readReturn}

\EndPhase
\Statex \}
\Statex

\START[upon receive]{ (\FWD,$\RVal_{i}$,$\Vals_{i}$,ts) from server $\ps{i}$}
\State $\fwd[i]\gets \RVal_{i}$
\State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
\EndPhase

\Statex
\START[upon receive]{ (\TS,$\ps{i}$,ts) from server $\ps{i}$}
\START[if] {$\phase=R2\lor\phase=R1$}
\State $\collectedTs[i]\gets ts$
\EndPhase
\START[if] {$\phase=R2$}
\State{\tiny $\smallestTimestamp \gets min(\{ts\in \collectedTs$ $|$ $\notOld(ts)=true\})$} \label{line:async:notOld}
% \Comment{There is no write operation that terminates for a timestamp $t'>\smallestTimestamp$.}
\START[for] $i \in  [1,n]$ $send(\getval,\smallestTimestamp)$ to server $\ps{i}$
\label{line:async:sendGetVal}
\EndPhase
\EndPhase
\EndPhase

\Statex

\START[upon receive]($\VALS$,$\Vals_{i},\shareTs$) from server $\ps{i}$
\START[if] {$\phase=R2$}
\State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
\State $\collectedTsShare[s]\gets \shareTs$
\State $\collectedShares_r[s]\gets \collectedShares_r[s]\cup \Vals.share$
\EndPhase
\EndPhase

\end{algorithmic}
}
\caption{Read operation of \algAsyncRBSign\, solution. Reader side.}
\label{alg:async:AtomicRegisterClientRead}
\end{figure}




\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]

\Statex

\START[Audit()]\{
\Statex $\collectedLog[i] \gets \emptyset, \forall i \in [1,n] $
\START[for] $i \in  [1,n]$ $send(\AuditReq)$ to server $\ps{i}$
\label{line:async:auditRequest}
\EndPhase
\START[repeat]
\State // Wait responses
\EndPhase
\State \textbf{until}$ |\{i:\collectedLog[i]\not=\emptyset\}|\geq n-f$
\label{line:async:waitAuditResponse}
\START[for] \textbf{all}$(\pr)\in \bigcup_{i\in[1,n]}\collectedLog[i]$ \textbf{do}
% \START[for] \textbf{all} $(\pr,v,wsn,rsn)$ with wsn the greatest sequence number
\State{\textbf{for} $1\leq k\leq n$ \textbf{do if} $(\pr)\in \collectedLog[k]$ \Statex
        \hfill \textbf{then} $\mathcal{E}_{\pr}\gets\mathcal{E}_{\pr}\cup\{k\} $}
\State{\textbf{if} $|\mathcal{E}_{\pr}|\geq =t$ \textbf{then} $E_A\gets E_A\cup (\pr) $}
\label{line:async:conditionReportAudit}
% \EndPhase
\EndPhase
\State{\textbf{return} $E_A$} 
% \Comment{For the accountability use sign message}

\EndPhase
\Statex \}

\START[upon receive] ($\AuditResp, \Logi$) from server $\ps{i}$
\State $\collectedLog[i]\gets \Logi$
\EndPhase

\end{algorithmic}
}
\caption{Audit operation of \algAsyncRBSign\, solution.}
\label{alg:async:AtomicRegisterClientAudit}
\end{figure}

% \begin{figure}[!htpb]
% {\footnotesize
% \begin{algorithmic}[1]

% \Statex

% \START[Audit()]\{
% \Statex $\collectedLog[i] \gets \emptyset, \forall i \in [1,n] $
% \START[for] $i \in  [1,n]$ $send(\AUDIT)$ to server $\ps{i}$
% \label{line:async:auditRequest}
% \EndPhase
% \START[repeat]
% \State // Wait responses
% \EndPhase
% \State \textbf{until}$ |\{i:\collectedLog[i]\not=\emptyset\}|\geq n-f$
% \label{line:async:waitAuditResponse}
% \START[for] \textbf{all}$(\pr,\langle ts\rangle)\in \bigcup_{i\in[1,n]}\collectedLog[i]$ \textbf{do}
% % \START[for] \textbf{all} $(\pr,v,wsn,rsn)$ with wsn the greatest sequence number
% \State{\textbf{for} $1\leq k\leq n$ \textbf{do if} $(\pr,\langle ts \rangle)\in \collectedLog[k]$ \Statex
%         \hfill \textbf{then} $\mathcal{E}_{\pr,ts}\gets\mathcal{E}_{\pr,ts}\cup\{k\} $}
% \State{\textbf{if} $|\mathcal{E}_{\pr,ts}|\geq f+1=t$ \textbf{then} $E_A\gets E_A\cup (\pr,ts) $}
% \label{line:async:conditionReportAudit}
% % \EndPhase
% \EndPhase
% \State{\textbf{return} $E_A$} 
% % \Comment{For the accountability use sign message}

% \EndPhase
% \Statex \}

% \START[upon receive] ($\AUDIT, \Logi$) from server $\ps{i}$
% \State $\collectedLog[i]\gets \Logi$
% \EndPhase

% \end{algorithmic}
% }
% \caption{Audit operation of \algAsyncRBSign\, solution.}
% \label{alg:async:AtomicRegisterClientAudit}
% \end{figure}





==> Legacy/algorithmsLegacy/asynchronousCase/auditServerAsyncUnbound.tex <==
\begin{figure}[!htpb]
{
\footnotesize
\begin{algorithmic}[1]
\Statex Initialization
\Statex $\Rts_{i} \gets  0$
\Statex $\RVal_{i} \gets \emptyset$
% \Statex $\RValblock \gets \emptyset$
\Statex $\Logi \gets \emptyset$
\Statex $\READERS_{i} \gets \emptyset$

\label{line:async:unbound:init}

\Statex

\Statex // Write Protocol Messages
\Comment{Pseudo code for server i}

% \Statex 
\START[upon \texttt{receive}] ($\writets,ts,[b_1,\ldots,b_n]$) from writer $\pw$
\label{line:async:unbound:receiveWriteVal}
\State $\RVal_{i} \gets \RVal_{i} \cup (b_{i},ts)$
\label{line:async:unbound:updateRValWriteVal}
\START[if] {$\Rts_{i}<ts$}
\{$\Rts_{i} \gets ts$\}
\label{line:async:unbound:updateRts}
\EndPhase
\State \texttt{\textbf{send}} $\writetsack$ to $\pw$
\label{line:async:unbound:writeAck}
\EndPhase
% \Statex

% \START[on receive] ($\getReaders$,ts) from reader $\pr$ 
% \State send($\sendReaders$,$\READERS_{i}$,ts) to $\pr$
% \label{line:async:unbound:concurrentReaderServer}
% \EndPhase

\Statex

\Statex // Read Protocol Messages
\START[upon \texttt{receive}] ($\getts,\nSeq$) from reader $\pr$
\State{\texttt{\textbf{send}}($\TS,\Rts,\nSeq)$)}
\label{line:async:unbound:sendTs}
\EndPhase

\Statex 

\START[upon \texttt{receive}] ($\GetValUnbound,ts,\nSeq $) from reader $\pr$
% \START \textcolor{red}{($\checkSignature(ts,\pw) = true$)}
\START[wait for] ($\Rts \geq ts )$
\label{line:async:unbound:waitTsSendTs}
\State \texttt{\textbf{send}}($\SendValUnbound,ts,\nSeq$) to $\pr$
\label{line:async:unbound:sendTs2}
\EndPhase
\EndPhase



\Statex

% \START[on receive] $(\GetSignature,ts)$ from reader $\pr$ \label{line:async:receiveGetSignature}
% \START \textcolor{red}{($\checkSignature(ts,f+1) = true$)}
% \State $\Logi \gets \Logi\cup \langle \pr,ts,\textcolor{red}{\sigma_{\pr}(\pr,ts)} \rangle$
% \label{line:async:unbound:logServRval}
% \State send($\GetSignatureAck,\signMessage{ts,\pr}{\ps{i}}$) to $\pr$
% \EndPhase
% \EndPhase

\START[upon \texttt{receive}] $(\GetBlocks,(\pr,ts,\nSeq)_{\sigma(\pr)})$ from reader $\pr$
\label{line:async:unbound:receiveGetBlocks}
% \START \textcolor{red}{($\checkSignature(ts,2f+1) = true$)}
\START[wait for] $\Rts\geq ts$
\label{line:async:unbound:waitTsSendVal}
\State $\Logi \gets \Logi \cup
(\pr,ts,\nSeq)_{\sigma(\pr)}$
\label{line:async:unbound:logServRval}
\State \texttt{\textbf{send}}($\SendBlock,\RVal[ts],\nSeq$) to $\pr$
\label{line:async:unbound:sendVal}
\EndPhase
\EndPhase

\Statex

\Statex // Audit protocol Messages
\START[upon \texttt{receive}] ($\AuditReq$) from owner $\pR$ of R 
\State \texttt{\textbf{send}}($\AuditResp$,$\Logi$) to $\pR$
\label{line:async:unbound:senLog}
% \State $\Log \gets \emptyset$
% \Comment{Audit operation is performed by correct and detect operation between two audit operation, be careful to not lose any information with concurrent read operation}

\EndPhase
\Statex

\end{algorithmic}{}
}
\caption{Pseudo-code at server $\ps{i}$.}
\label{alg:async:unbound:AtomicRegisterServer}
\end{figure}{}



==> Legacy/algorithmsLegacy/asynchronousCase/auditServerSave.tex <==
\begin{figure}[!htpb]
{
\footnotesize
\begin{algorithmic}[1]
\Statex Initalization
\Statex $\Rts_{i} \gets  0$
\Statex $\RNextVal_{i} \gets \langle \perp, \perp, \perp \rangle$
\Statex $\RVal_{i} \gets  \langle \perp, \perp, \perp \rangle$
\Statex $\RPrev_{i} \gets  \langle \perp, \perp, \perp \rangle$
\Statex $\RPrevTwo_{i} \gets  \langle \perp, \perp, \perp \rangle$
% \Statex $\RValblock \gets \emptyset$
\Statex $\Logi \gets \emptyset$
\Statex $\READERS_{i} \gets \emptyset$

\label{line:async:init}

\Statex

\Statex // Write Protocol Messages
\Comment{Pseudo code for server i}
\START[on receive] ($\nextval,\langle ts,b \rangle$) from writer $\pw$
% \State $\RValblock[ts] \gets b$
\State $\RNextVal_{i} \gets \langle ts,b\rangle$
\label{line:async:updateRNextVal}
% \State $\RShare\_wb[ts] \gets sh_{wb}$
% \label{line:async:UpdateRShare}
% \State $\RNextWBsecret \gets \RNextWBsecret\cup sh $
% \label{line:async:UpdateRNextValsecrects}
% \State $\RNextWBproof \gets \RNextWBproof\cup pr$
% \label{line:async:UpdateRNextValproofs}
\State send $\nextvalack$ to $\pw$
\label{line:async:writeAck1}
\EndPhase

% \Statex 

\START[on receive] ($\writeval$) from writer $\pw$
\label{line:async:receiveWriteVal}
% \State $\RVal \gets \RVal\cup\RNextVal$
% \label{line:async:UpdateRValWriteVal}

\State $\RPrev2_{i} \gets \RPrev_{i}$
\label{line:async:updateRPrev2WriteVal}
\State $\RPrev_{i} \gets \RVal_{i}$
\label{line:async:updateRPrevWriteVal}
\Comment{Used if the writer crash before sending the list of concurrent readers to servers}
\State $\RVal_{i} \gets \RNextVal_{i}$
\label{line:async:updateRValWriteVal}

% \State $\RValsecrets \gets \RValsecrets\cup\RNextWBsecret$
% \label{line:async:UpdateRValsecrectsWriteVal}
% \State $\RValproofs \gets \RValproofs\cup\RNextWBproof$
% \label{line:async:UpdateRValproofsWriteVal}
\State send $\writevalack$ to $\pw$
\label{line:async:writeAck2}
% \State $\Log \gets \langle r,\RVal,\RPrev,timer,\writeval\rangle$ 
\EndPhase

% \Statex

\START[on receive] ($\writets,ts,\CR$) from writer
\START[if] {$\Rts_{i}<ts$}
\label{line:async:writetsRts}
\State $\Rts_{i} \gets ts$
\label{line:async:updateRts}
\EndPhase
\START[for each] $\pr\in \CR$
\label{line:async:concurrentReaderServerOperation}
\State $\Logi \gets \Logi\cup \langle id(\pr),ts \rangle$
\label{line:async:logServFwd}
\State $send(\FWD,\RVal_{i},\{\RVal_{i},\RPrev_{i},\RPrevTwo_{i}\})$ to $\pr$
\label{line:async:forwardToReader}
\EndPhase
\State{$\READERS_{i} \gets \READERS_{i} \smallsetminus \CR$}
\label{line:async:removeConcurrentReaderDetection}
\State send $\writetsack$ to $\pw$
\label{line:async:writeAck3}
\EndPhase
% \Statex
\START[on receive] ($\getReaders$,ts) from reader $\pr$ 
\State send($\sendReaders$,$\READERS_{i}$,ts) to $\pr$
\label{line:async:concurrentReaderServer}
\EndPhase

\Statex

\Statex // Read Protocol Messages
\START[on receive] ($\getts$) from reader $\pr$
% \State $\Logi \gets \Logi\cup \langle id(\pr) \rangle$
% \label{line:async:logServ}
\State $\READERS_{i} \gets \READERS_{i}\cup \pr$
\label{line:async:addConcurrentReader}
\State{send($\TS,\ps,\Rts_{i}$)}
\EndPhase

% \Statex 

\START[on receive] ($\getval$,ts) from reader $\pr$
% \State $\Logi \gets \Logi\cup \langle id(\pr), ts \rangle$
% \label{line:async:logServ}
\START[wait for] ($\RVal_{i}.ts \geq ts)$
\label{line:async:waitTsSendVal}
% \State send($\VALS,\{\RVal_{i},\RPrev_{i},\RPrevTwo_{i}\}$, \Statex
%                 \hfill \{$encrypt(hash(\RVal_{i}.ts,\pr))_i,$ \Statex
%                 \hfill $encrypt(hash(\RPrev_{i}.ts,\pr))_i,$ \Statex
%                 \hfill $encrypt(hash(\RPrevTwo_{i}.ts,\pr))_i\}$) to $\pr$
\START[if] ($\RVal_{i}.ts = ts)$
\State $\Logi \gets \Logi\cup \langle \pr,ts \rangle$
\label{line:async:logServRval}
\State send($\VALS,\{\RVal_{i},\RPrev_{i},\RPrevTwo_{i}\}$, \Statex
                \hfill \{$encrypt(hash(\RVal_{i}.ts,\pr))_i,$
\label{line:async:sendRVal}

\EndPhase
\START[if] ($\RPrev_{i}.ts = ts)$
\State $\Logi \gets \Logi\cup \langle \pr,ts \rangle$
\label{line:async:logServRPrev}
\State send($\VALS,\{\RVal_{i},\RPrev_{i},\RPrevTwo_{i}\}$, \Statex
                \hfill $encrypt(hash(\RPrev_{i}.ts,\pr))_i,$ 
\label{line:async:sendRPrev}

\EndPhase
\START[if] ($\RPrevTwo_{i}.ts = ts)$
\State $\Logi \gets \Logi\cup \langle \pr,ts \rangle$
\label{line:async:logServRPrevTwo}
\State send($\VALS,\{\RVal_{i},\RPrev_{i},\RPrevTwo_{i}\}$, \Statex
                \hfill $encrypt(hash(\RPrevTwo_{i}.ts,\pr))_i\}$) to $\pr$
\label{line:async:sendRPrevTwo}
\EndPhase  

\label{line:async:sendVal}

\EndPhase
% \START[Else If $\RPrev.ts = ts $]
% \State send(\VALS,$\RPrev$) to r
% \EndPhase
% \START[Else If $\RPrevTwo.ts = ts $]
% \State send(\VALS,$\RPrevTwo$) to r
% \Comment{Need a scenario to see if sending $\RPrevTwo$ is required}
% \label{line:async:SendVal}
% \EndPhase

\EndPhase

% \Statex


\START[on receive] ($\wbackval$,ts,$\collectedTsShare$) from reader $\pr$
\START[wait for] ($\RNextVal_{i}.ts \geq ts)$
\label{line:async:wback1WaitRNextVal}
\START[If] $\RNextVal_{i}.ts = ts$ \Statex
    \hfill $\land consistent(f+1,ts,\collectedTsShare)$
\label{line:async:conditionWB1}
% \Comment{At least 1 correct has ts in $\RVal$}
\State $\RPrev2_{i} \gets \RPrev_{i}$
\label{line:async:updateRPrev2WBack}
\State $\RPrev_{i} \gets \RVal_{i}$
\label{line:async:updateRPrevWBack}
\State $\RVal_{i} \gets \RNextVal_{i}$
\label{line:async:updateRValWBack}
\EndPhase
%\State send(\wbackvalack) to r
\EndPhase
\EndPhase

\START[on receive] $(\wbackts,ts,\collectedTsShare)$ from reader $\pr$ \label{line:async:receiveWbTs}
\START[wait for] ($\RNextVal_{i}.ts \geq ts)$
\label{line:async:wbakcWaitRNextVal}
\START[If] $\Rts_{i} < ts \land consistent(2f+1,ts,\collectedTsShare)$]
\label{line:async:conditionWriteBackTs}
\Comment{True for correct reader}
\State{$\Rts_{i} \gets ts$}
\label{line:async:writebacktsRts}
\EndPhase
\START[If] $\Rts_{i} \geq ts$
\label{line:async:writebacktsRtsGreater}

\State{$\READERS_{i} \gets \READERS_{i} \smallsetminus \pr$}
\label{line:async:removeConcurrentReaderEndRead}
\State send($\wbacktsack$) to $\pr$
\label{line:async:writebackTsAck}

\EndPhase

\EndPhase
\EndPhase
\Statex


\Statex // Audit protocol Messages
\START[on receive] ($\AuditReq$) from owner $\pR$ of R 
\State send($\AuditResp$,$\Logi$) to $\pR$
\label{line:async:senLog}
% \State $\Log \gets \emptyset$
% \Comment{Audit operation is performed by correct and detect operation between two audit operation, be careful to not lose any information with concurrent read operation}

\EndPhase
\Statex

% \START[on receive] (WBACK,$ts,Shares$)from reader r
% % \START[if] {$\RPrev$.ts$\geq$ts}
% % % \State send(WBACK\_VAL\_ACK) to r
% % \EndPhase
% \START[if]{ $\RVal.ts\geq ts$}
% % \State $\RPrev2 \gets \RPrev$
% % \label{line:async:UpdateRPrev2WBack}
% % \State $\RPrev \gets \RVal$
% % \label{line:async:UpdateRPrevWBack}
% % \State $\RVal \gets \RNextVal$
% \label{line:async:ConditionWBack}
% \EndPhase

% \START[else if]{ $\RNextVal.ts=ts \land  consistent(Shares,\RNextVal.sh)$}
% \label{line:async:ConditionConsintentWBack}

% \State $\RPrev2 \gets \RPrev$
% \label{line:async:UpdateRPrev2WBack}
% \State $\RPrev \gets \RVal$
% \label{line:async:UpdateRPrevWBack}
% \State $\RVal \gets \RNextVal$
% \label{line:async:UpdateRValWBack}
% \EndPhase

% \EndPhase

\end{algorithmic}{}
}
\caption{Server side of \algAsyncRBSign\, solution.}
\label{alg:async:AtomicRegisterServer}
\end{figure}{}



==> Legacy/algorithmsLegacy/synchonousCase/auditClient.tex <==

\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]

\Statex Initialization
\Statex $ ts \gets 0$

\Statex

\START[Write](v)\{

\State{$ts \gets ts+1$} \label{line:audit:incts}
\State{$[b_1,\ldots,b_n]\gets generateBlocks()$}

\Statex{// Phase W1 Round 1}
\START[for] $i \in [1,n]$ $send(\nextval,b_i,ts,sh_i)$ to server $s_i$
\label{line:audit:nextVal}
\EndPhase
\State{ $wait(\delta)$}
\label{line:audit:nextValWait}


\Statex // Phase W2 Round 2
\START[for] $i \in [1,n]$ $send(\writeval)$ to server $s_i$
\label{line:audit:writeVal}
\EndPhase
\State{ $wait(\delta)$}

\State{return}
\EndPhase
\Statex \}

\Statex
\Statex

\START[Read()]\{
\Statex $\forall i,\, \collectedValues[i] \gets \emptyset$
\Statex $\possibleVal \gets \emptyset$
\Statex $\writtenBackVal \gets \langle \perp,\perp\rangle$

\Statex

\Statex // Phase R1 Round 1
\START[for] $i \in  [1,n]$ $send(\getval)$ to server $i$
\EndPhase
\State{$wait(2\delta)$}
% \START[repeat] \{



% \EndPhase 
% \State \} until $\exists(v,ts): |\{s:\langle v,ts,-\rangle \in collected\_values[s]\}|\geq 2f+1=\tau$
\label{line:audit:Condition}
\State{$\possibleVal \gets$ $\{\langle v,ts\rangle:|\{s:\langle v,ts,-\rangle = collected\_values[s]\}|\geq 2f+1=\tau\}$}
\label{line:audit:possibleVal}
\Comment{Use a function consistent or validity}

\Statex
\Statex // Phase WB1 Round 2
\State{$\writtenBackVal$  $\gets \{\langle v,ts\rangle \in  \possibleVal: \forall \langle v',ts'\rangle \in  \possibleVal, ts \geq ts'\}$}
\label{line:audit:writtenBackEQPossibleVal}
\State{$Shares \gets GetShares(\writtenBackVal,collected\_values)$}
\START[for] $i \in  [1,n]$ send($WBACK,\writtenBackVal.ts,Shares$) to server $s_i$
\label{line:audit:WritteBackts}
\State{ $wait(\delta)$}

\EndPhase

\State return \writtenBackVal

\EndPhase
\Statex \}
\Statex
\START[When] (VALS,$\langle v,ts,sh\rangle,\langle v',ts',sh'\rangle$)  received from server $i$
\State{\textbf{then}} $\collectedValues[i]\gets \langle(v,ts,sh),(v',ts',sh')\rangle$ \label{line:audit:ValsMessage}

\Comment{Message handler}
\EndPhase

\Statex
\Statex

\START[Audit()]\{
\Statex $\forall i, \collectedLog[i] \gets \emptyset$
\START[for] $i \in  [1,n]$ $send(AUDIT)$ to server $i$
\label{line:audit:auditRequest}
\EndPhase
\State $wait(2\delta)$
\label{line:audit:audit2delta}
\START[if] (AUDIT,$ Log_i$) received from server $i$ \textbf{then} 
\State $\collectedLog[i]\gets Log_i$
% \State $\collectedLog[i]\gets \langle p_r,\RPrev\rangle$
\EndPhase

\START[for] \textbf{all}$(p_r,\langle v,ts,- \rangle)\in \bigcup_{i\in[1,n]}\collectedLog[i]$ \textbf{do}
% \START[for] \textbf{all} $(p_r,v,wsn,rsn)$ with wsn the greatest sequence number
\State{\textbf{for} $1\leq k\leq n$ \textbf{do if} $(p_r,\langle v,ts,- \rangle)\in Log[k]$ \textbf{then} $\mathcal{E}_{p_r,v}\gets\mathcal{E}_{p_r,v}\cup\{k\} $}
\State{\textbf{if} $|\mathcal{E}_{p_r,v}|\geq f+1=t$ \textbf{then} $E_A\gets E_A\cup (p_r,v) $}
% \EndPhase
\EndPhase
\State{\textbf{return} $E_A$} 

\EndPhase
\Statex \}

\end{algorithmic}
}

\caption{\algSyncSign client side}
\label{alg:SyncAuditableAtomicRegisterClient}
\end{figure}





==> Legacy/algorithmsLegacy/synchonousCase/auditServer.tex <==
\begin{figure}[!htpb]
{\footnotesize

\begin{algorithmic}[1]
\Statex Initalization
\Statex $\RNextVal \gets \langle \perp,0,\perp\rangle$
\Statex $\RVal \gets \langle \perp,0,\perp\rangle$
\Statex $\RPrev \gets \langle \perp, 0, \perp\rangle$
\Statex $\Logi \gets \emptyset$
\label{line:audit:init}

\Statex

\Statex Pseudo code for server i
\Statex // Write Protocol messages
\START[on receive] ($\nextval,\langle v,ts,sh \rangle)$ from writer
\State {$\RNextVal$ $\gets \langle v, ts, sh \rangle$}
\label{line:audit:RNextVal}
\EndPhase


\Statex

\START[on receive] (\writeval) from writer
% \State $\RPrev2 \gets \RPrev$
% \label{line:audit:UpdateRPrev2WriteVal}
\State $\RPrev \gets \RVal$
\label{line:audit:UpdateRPrevWriteVal}
\State $\RVal \gets \RNextVal$
\label{line:audit:UpdateRValWriteVal}


% \State $\Log \gets \langle r,\RVal,\RPrev,timer,\writeval\rangle$

\EndPhase

\Statex
\Statex

\Statex // Read Protocol Message

\START[on receive] (\getval) from reader r
\State $\Logi \gets Log\cup \langle r,\RVal,\RPrev \rangle$
\label{line:audit:logServ}
\State send(VALS,$\RVal$,$\RPrev$) to r
\label{line:audit:SendVal}

\EndPhase
\Statex

\START[on receive] (AUDIT) from owner $p_R$ of R 
\State send(AUDIT,$Log$) to $p_R$
\label{line:audit:SenLog}
% \State $\Log \gets \emptyset$
% \Comment{Audit operation is performed by correct and detect operation between two audit operation, be careful to not lose any information with concurrent read operation}

\EndPhase
\Statex

\START[on receive] (WBACK,$ts,Shares$)from reader r
% \START[if] {$\RPrev$.ts$\geq$ts}
% % \State send(WBACK\_VAL\_ACK) to r
% \EndPhase
\START[if]{ $\RVal.ts\geq ts$}
% \State $\RPrev2 \gets \RPrev$
% \label{line:audit:UpdateRPrev2WBack}
% \State $\RPrev \gets \RVal$
% \label{line:audit:UpdateRPrevWBack}
% \State $\RVal \gets \RNextVal$
\label{line:audit:ConditionWBack}
\EndPhase

\START[else if]{ $\RNextVal.ts=ts \land  consistent(Shares,\RNextVal.sh)$}
\label{line:audit:ConditionConsintentWBack}

% \State $\RPrev2 \gets \RPrev$
% \label{line:audit:UpdateRPrev2WBack}
\State $\RPrev \gets \RVal$
\label{line:audit:UpdateRPrevWBack}
\State $\RVal \gets \RNextVal$
\label{line:audit:UpdateRValWBack}
\EndPhase
\EndPhase
\end{algorithmic}{}
}

\caption{\algSyncSign server side}
\label{alg:SyncAuditableAtomicRegisterServer}
\end{figure}{}







==> Legacy/consensusNumber.tex <==

\subsection{Consensus with two processes}

The following algorithm using Strong Auditable Atomic Register solves the consensus.

\input{CaseUnbound/algorithms/consensusNumberTwoAlg}

\begin{lemma}
\label{lemma:async:consensusNumberTwo}
Algorithm Figure \ref{alg:async:consensusTwoProcess} solves consensus for two processes

\end{lemma}\spaceLemmaProof

\begin{proofL}
We prove this by exploring exhaustively all the different possible scenario. We consider two different processes, $p_0$ and $p_1$. We denote all the possible different operations.
\begin{enumerate}
    \item $p_0$ write $R_{p_0}$
    \item $p_0$ read $R_{p_1}$
    \item $p_0$ audit $R_{p_0}$    \item $p_1$ write $R_{p_1}$
    \item $p_1$ read $R_{p_0}$
    \item $p_1$ audit $R_{p_1}$
\end{enumerate}
The table Figure \ref{table:consensusNumberTwo} list all the possible scenario. The scenario 123456 correspond to the scenario where operation 1 ($p_0$ write $R_{p_0}$) happens first, then 2 ($p_0$ read $R_{p_1}$), then 3 ($p_0$ audit $R_{p_0}$), then 4 ($p_0$ write $R_{p_1}$), then 5 ($p_0$ read $R_{p_0}$), and finally 6 ($p_0$ audit $R_{p_1}$).
\end{proofL}

\begin{figure}[!ht]
\centering
    \includegraphics[scale=0.575]{image/consensusNumber.PNG}
    \caption{Scenarios consensus two process}
    \label{table:consensusNumberTwo}
\end{figure}

\subsection{Consensus with n processes}
If we consider that a Strong Auditable Atomic Register, (SAAR) $R{p_i}$ owned by process $p_i$ can only be audited by process $p_i$, then SAAR has consensus number two.

\begin{lemma}
\label{lemma:async:consensusNumberTwo}
There is no algorithm that uses only SAAR (auditable register that can be audited only by a single process) that solves consensus for three processes.
\end{lemma}\spaceLemmaProof

\begin{proofL}
The idea of the proof follow the classic idea of the impossibility proof to solves consensus with two processes using only auditable register.

Suppose that algorithm $\mathcal{A}$ solves the consensus. Then $\mathcal{A}$ can be run until it reaches a critical state s. 
We consider three processes A, B and C. Suppose A's next move carries the protocol to a 0-valent state, and B's as C’s next move carries the protocol to a 1-valent state (If not, then swap thread names.) What methods could A, B or C be about to call? We now consider an exhaustive list of the possibilities: one of them reads from a register, they all write to separate registers, (or they both write to the same register (if we consider multi writer single auditor register).
Suppose A is about to read a given register (B may be about to either read, write or audit the same register or a different register). In the first scenario, B moves first, driving the protocol to a 1-valent state s', and then B runs solo and eventually decides 1. In the second scenario, C moves first driven the protocol to a 1-valent state s". In the third execution scenario, A moves first, driving the protocol to a 0-valent state, and then B  takes a step to reach state s" (if not swap B and C names). 
% B then runs solo starting in s’ and eventually decides 0 (same C). The problem is that the states s′ and s″’ are indistinguishable to C (the read A performed could only change its thread-local state, and be either visible to B or be visible to C, but this read operation can not be visible to both B and C), which means that B or C must decide the same value in both scenarios, a contradiction.

\end{proofL}

\input{diagram/impossibilityConsensus3process}

If we consider now a Strong Multi Auditable Atomic Register, (SMAAR) $R{p_i}$ owned by process $p_i$, that can only be written by $p_i$, and can be audited by all processes, then SMAAR can solve consensus for any number of processes. Note that such a register is not more costly to obtain than a SAAR, and that algorithm presented Figure \ref{alg:async:unbound:AtomicRegisterClientWrite}, \ref{alg:async:unbound:AtomicRegisterClientRead}, and \ref{alg:async:unbound:AtomicRegisterServer} almost respect the SMAAR specification. (It just would require  that the function Audit() (line \ref{line:async:unbound:auditStart} to \ref{line:async:unbound:auditEnd} algorithm \ref{alg:async:unbound:AtomicRegisterClientWrite}) to be executable by all the processes and not only by the writer)

\input{CaseUnbound/algorithms/consensusNumberN}


==> Legacy/consensusNumberN.tex <==

\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Definitions:}
\Statex $\Pi$ the set ${p_1,...,p_n}$ of all the processes  in the system 
\Statex  $R_{p_{i_{i\in[1,n]}}}$ Strong Auditable Atomic Register owned by process $p_{i}$ 
% \Statex  $R_{p_j}$ Strong Auditable Atomic Register owned by process $p_{j}$
\Statex
\Statex \textbf{Initialization :}
\Statex $v_0 \gets random(0,1)$
\Statex $value_{read} \gets \emptyset$
\Statex $value_{audit} \gets \emptyset$
\Statex
\START[consensus($v_0$)]
\State{write($R_{p_i},v_0$)}
\START[For ]{$p\in \Pi$}
    \State{$value_{read} \gets value_{read}\cup read(R_{p_j})$}
\EndPhase
\START[For ]{$p\in \Pi$}
    \State{$value_{audit} \gets value_{audit} \cup audit(R_{p_i})$}
\EndPhase
\State{return {\sf selectValue}($v_0, value_{read}, value_{audit})$}
\EndPhase

\Statex

% \START[selectValue($v_0, value_{read}, value_{audit}$)]
% \START[if] {$value_{read} = \perp$}
% \State{return $v_0$}
% \EndPhase
% \START[if] {$value_{audit}= \{p_j,\perp\}$}
% \State{return $value_{read}$}
% \EndPhase
% \START[if] {$p_i<p_j$}
% \State{return $value_{read}$}
% \EndPhase
% \START[if] {$value_{audit}= \perp AND\, p_i>p_j$}
% \State{return $v_0$}
% \EndPhase
% \START[if] {$value_{audit}= \{p_j,v_0\} AND\, p_i>p_j$}
% \State{return $v_0$}
% \EndPhase

% \EndPhase



\end{algorithmic}
}
\caption{Pseudo-code to solves consensus for n processes.}
\label{alg:async:consensusTwoProcess}
\end{figure}


==> Legacy/consensusNumberTwoAlg.tex <==

\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Definitions:}
\Statex  $R_{p_0}$ Strong Auditable Atomic Register owned by process $p_{0}$ 
\Statex  $R_{p_1}$ Strong Auditable Atomic Register owned by process $p_{1}$
\Statex Pseudo code for process $p_i$
\Statex
\Statex \textbf{Initialization :}
\Statex $v_i \gets random(0,1)$
\Statex $value_{read} \gets \perp$
\Statex $value_{audit} \gets \perp$
\Statex
\START[propose($v_i$)]
\State{write($R_{p_i},v_i$)}
\State{$value_{read} \gets read(R_{p_j})$}
\State{$value_{audit} \gets audit(R_{p_i})$}
\State{return {\sf selectValue}($v_i, value_{read}, value_{audit})$}
\EndPhase

\Statex

\START[selectValue($v_0, value_{read}, value_{audit}$)]
\START[if] {$value_{read} = \perp$}
\State{return $v_i$}
\EndPhase
\START[if] {$value_{audit}= \{p_j,\perp\}$}
\State{return $value_{read}$}
\EndPhase
\START[if] {$p_i<p_j$}
\State{return $value_{read}$}
\EndPhase
\State{return $v_i$}
% \START[if] {$value_{audit}= \perp AND\, p_i>p_j$}
% \State{return $v_0$}
% \EndPhase
% \START[if] {$value_{audit}= \{p_j,v_0\} AND\, p_i>p_j$}
% \State{return $v_0$}
\EndPhase




\end{algorithmic}
}
\caption{Pseudo-code to solves consensus for two processes.}
\label{alg:async:consensusTwoProcess}
\end{figure}



==> Legacy/discussion.tex <==
If there is collaboration between the different Byzantine readers that can cooperate and communicates with each other, we need to make the readers prove it contact enough servers asking for a specific value $v$ before the servers send the block for the value $v$ to the readers.

This can be done by increasing the number of round. After a reader receives sufficiently many value that make him sure to read value for timestamp ts. It has to send to the servers that it will be reading the value ts. And finally send a final message that prove that enough servers are well aware that it will be reading value for timestamp $ts$, and it is just to this message that servers can send the block to the reader.



So a solution for the Strong accuracy could work as follow.
\begin{itemize}
    \item 1st Phase,
        the reader asks for the timestamp.
 
    \item 2nd Phase,
        The reader sends a 'GET VAL' message for the smallest timestamp (greater than $2f+1$ others).
        Then servers send back this timestamp with a signature.
    
    \item 3rd
        When the reader collects $f+1$ responses for the same timestamp, the reader create the corresponding BLS signature with all the response of the servers and send the timestamp with the BLS signature to all the servers
        The servers, if the BLS is correct, add the reader in their log and acknowledge the reader with a signature
    
    \item 4th
        The reader creates a new BLS signature with $2f+1$ acks of the servers and send it with the timestamp $ts$ to the servers. The servers send their block corresponding to timestamp ts.
    
\end{itemize}

Notice that it should be possible to merge phase 3 and 4 by implementing a reliable broadcast between the reader and servers.

We need two more round of communication after phase 2 because the $GetVal(ts)$ message send by the reader in the phase 2 cannot be use as a proof that the reader will read the value with timestamp $ts$. Indeed, it is possible that $ts$ send in this message by the reader has only be received by Byzantine process. Then the reader have to wait response for GetVal message, and if it receive $2f+1$ message for a same value, now it is sure that all correct servers will eventually have the block (due to reliable broadcast) and it can send the message to notify that it will read the value, (then being add in the log at this moment) and finally ask for the blocks, with the proof that sufficiently many servers are aware that the reader is reading for this value.

(With reliable broadcast between server and reader, that could be done with less round, by making the server respond after it forward the proof to other servers)

==> Legacy/impossibilityStrong.tex <==

\begin{lemma}
For a reader to read a value $v$ with $\tau\geq 2f+1$ then at least $2f+1$ correct servers must have received messages from the write operation that have written $v$.
\end{lemma}


\begin{proofL}
If the reader needs $\tau$ blocks to read the data, then at least $\tau$ correct servers must send it to the reader.  For a correct server to send the block to the reader, it must have received first the messages for this write operation from the writer.

Note that it is also possible that the reader read the value $v$ with the cooperation of Byzantine servers, but to ensure the termination, only correct servers can be taken into account.
\end{proofL}

\begin{lemma}
At the end of a write operation, (only) at least $f+1$ correct servers have received messages from the writer.
\end{lemma}

\begin{proofL}
As the write operation is wait free, we cannot wait for more than $2f+1$ acknowledgment. As there is $f$ byzantine, we can only assure that $f+1$ correct servers are aware of the write operations and received messages from the writer.
\end{proofL}

\begin{proofL}
Proof by contradiction, assume that a  bounded  asynchronous  regular  register algorithm exists.

Then, all read terminates in respect to the regular semantics. Assume that process $p$ read value $v$, then process $p$ receive $2f+1$ blocks for value $v$ (by definition $\tau=2f+1$). For all bounded algorithm (space/\textit{complexity}), the reader $p$ must have received those blocks in response to a request messages. Furthermore, those 2f+1 blocks must have been sent by correct processes.
Note the following two statement, (i) at the end of a write operation $\op{w}$, in the worst case scenario at most $n-2f=f+1$ correct process received messages for $\op{w}$, (ii) a server can send a block for value v to the reader, only if it received first messages from the writer for value v.

Then, from those two statement, we can see, that for all algorithm, process p can terminates only if all correct servers received first messages from the a same write operation, and then that all correct servers answer to the read request.

Assume the following scenario. We divide all the server in three group of processes, $Q_1$ with $|Q_1|=f$, that are late correct processes, $Q_2$ with $|Q_2|=f+1$ correct processes that make write progress and $Q_3$ with $|Q_3|=f$ the byzantine. Assume that when the read operation starts, the last write operation completed is $\op{w1}$, and that only process in $Q_2$ and $Q_3$ receive messages for this write operation. The last write operation that all correct processes are aware of is $\op{w0}$, assume that there is an unbounded number of write operation between $\op{w1}$ and $\op{w0}$ that only the correct process in $Q_2$ are aware of. We note this time $t_1$.

Now assume that when $Q_1$ will be aware of $\op{w1}$, let say at time $t_2$ then the last write operation is $\op{w2}$, with an unbounded number of write operation between $\op{w1}$ and $\op{w2}$. (with only correct of $Q_2$ that are aware of them). We note $t_3$, $t_4$ etc, for time with the same scheme.
Assume now that all correct servers receive messages at the same time. Then before $t_2$, it is impossible for $p$ get enough blocks for a correct values. Then, after $t_2$ it is possible for p to get all blocks for $v_1$. The issue there is that servers cannot wait a new read request from the reader, because with this kind of solution, this could result of an unbounded number of request from the reader to servers between $t_1$ and $t_2$. It cannot also come from the servers, because in this case, byzantine could make servers send new messages after each write operation between $t_1$ and $t_2$ which correspond to an unbounded number of messages. 


Assume the time $t_0$ the instant where all correct servers received messages for the last write operation before the read operation $v_0$, and $t_\infty$ the time of the last (concurrent) write operation for $v_\infty$. Between write operation $\op{v_0}$ and $\op{v_\infty}$ there is a potential infinite number of write operation. Eventually, $t_0>t_\infty$ such that when all correct servers receive messages for $v_0$, at least $f+1$ other servers received an unbounded number of other write operation. So if any of these $f+1$ correct servers receive messages from the reader after $t_\infty$ they won't never be able to send  the block corresponding to $v_0$. Then we can assume the existence of time $t_\infty+$, at which all correct servers receive messages for $v_\infty$, but in this case, if servers receive messages from the reader at $t_0$, then they would ask either to send a value new value at each concurrent write operation, which is then unbounded
\end{proofL}

\begin{proofL}
Idea of impossibility for Theorem \ref{theorem:async:imopssibilityBondedAudit}.

First let's study the case of safe register, where the impossible result doesn't stand.

Suppose a finite unbounded number of successive successful write operations, succeeded by a read operation $\op{r}$. 

As there is f byzantine, and that it is impossible to wait more than $n-f$ responses, it is possible that $f$ correct processes are not aware of any of the write operations when $\op{r}$ begins, and that it is only the $f$ byzantine in collaboration with $f+1$ correct system that make those write operation progress. 

Once $\op{r}$ occurs, the reader gets at most $f+1<\tau$ blocks from correct processes, and won't be able to read any value (the byzantine won't collaborate). What could give the termination, is that eventually, correct servers will catch up, and get messages from the writer for all write operations.

% When the $f$ late servers get messages from the writer, as there is an unbounded number of write operation.
Then there is a solution to provide safe semantics. The reader have to sent to servers the timestamp of the value it wish to read. The reader can do that when it gets $f+1$ responses from correct servers that participate to the last write operation. Then  the $f$ late servers, when they get the corresponding value will forward it to the reader.

Also the value decide must have a timestamp that is superior or equal to at least $2f+1$ timestamp. This is necessary to not decide late value cause of the byzantine that could made the reader ask for a value that does not correspond to the last write. 

The difference between safe and regular semantics, is the study in case of concurrent read operation with write operation. Lets now consider an unbounded number of write operation before $\op{r}$ begins but also on unbounded number write operation after $\op{r}$ begins. 

We still have $f$ correct servers that are late, and only $f+1$ correct processes that are making write operation progress (with the help of the byzantine). In this case, between the reception of the message from the reader and each correct server, an unbounded number of write operation could occur, such that it is impossible for the reader to agree on a specific one, and even if it does, between the moment the reader will resent a message to servers to ask this specific value, an unbounded number of write operation could occur that make impossible the server kept this information unless their memory is unbounded.
\end{proofL}

\begin{proofL}
IDEA of impossibility.

It seems impossible to have strong auditability in asynchronous model, with a bounded waitfree solution and safe register semantics. The idea is that to provide safe register semantics in presence of $f$ faulty servers, then at most $n-2f$ servers are needed to read the value.

Suppose that the information of $n-2f+1$ servers are needed to read the value $v$ written in operation $\op{w}$. Then, after the success write operation $\op{w}$, at least $n-2f+1$ servers must contain this information. Since the algorithm is wait free, at most $n-f$ answer from server can be wait at any time of the execution before going on the next phase. This means that $\op{w}$ could terminates by contacting only the sames $n-f$ servers. As there is $f$ byzantine, in the worst case, only $n-2f$ correct servers are reached during $\op{w}$. So only $n-2f$ servers have information about $v$ and write $\op{w}$, but $n-2f+1$ servers are needed to read a value, so it is impossible to read a value without the collaboration of a byzantine.

An idea could be to wait until all correct server are reached, which can eventually be the case. The issue of such a solution, is that an unbounded number of write operation could occur, which would ask to keep in memory an unbounded number of variables.

Lets do a scenario to understand.

Assume a write operation $\op{w}(v)$. Then as there is f byzantine and that the algorithm is waitfree, at most $n-f$ answer can be wait at any stage. Then we can assume that only $n-f$ are reached, and that f correct process are slow, and don't get the information about this read operation. Then a reader $p_r$ start a read operation. It can wait the response of only $n-f$ servers, and then potentially only get the response from $n-2f$ servers that have the information about the read operation. So if $p_r$ needs more than $n-2f+1$ information to read v, it cannot.

An other possible scenario, is that $p_r$ try to read v. First, $p_r$ gets the response from f servers that have the information. After what, all the other servers answer late. Then an unbounded number of write operation occurs. After what the reader get the response from $f+1$ other correct servers, and never gets more than $n-2f$ answer for the same value.
\renewcommand{\toto}{lemma:async:imopssibilityBondedAudit}
\end{proofL}

Is the issue remains about weak auditability ?

Not necessarily because we can imagine a mechanism to avoid the reader to ask the information of the $n-2f$ server to read if it does not first contact $n-f$ servers. The issue is that Theorem \ref{theorem:async:imopssibilityBondedAudit} shows that the information collected by contacting the $n-f$ servers (before contacting the $n-2f$ to read the value) cannot be value based. So the issue is that it seems possible for a reader to read a first value, and then to read a new one without being detected. This solution still allows to detect the first read operation of a reader. 



%%%%%%%%%%%%%% INTERESTING %%%%%%%%%%
\subsection{Other issue}
The kind of solution we use, with a number of blocks required to read a value, does not really protect against a coalition of reader, that could all on their own contact a single server (At less than f). In this case, strong accuracy is impossible to be achieved and weak accuracy required to sign messages.
%%%%%%%%%%%%%% INTERESTING %%%%%%%%%%

==> ToDo.tex <==

-- To prove impossibility of having a solution that guarantees Very Strong Accuracy and Completeness, with or without collusion (3f+1)

-- Does the impossibility remains (of having a solution that guarantees Very Strong Accuracy) with Eventual Completeness, with or without collusion (3f+1)


Solutions without and with collusion (the solution does not change with collusion):
 -- Strong Accuracy and Completeness (3f+1) Done
 -- Very Strong Accuracy and Completeness (4f+1) Done, does exist a solution for 3f+1? cf. first point on the impossibility

Solutions with and without collusion:
-- Eventual Completeness and Strong Accuracy. To do
-- Eventual Completeness and Very Strong Accuracy. To do

-- Safe register bound

---- Alex's todo -----


    1.	Formaliser la propriété de Very Strong Accuracy et proposer une implémentation (Bien finaliser la solution pour la Strong Accuracy puis la Very Strong)
2.	Étudier la prise en compte des écrivains Byzantins [1]
3.	Étudier l’adaptation du registre auditable au multi-writer case[1], et à d’autre objet distribué classique (compteur)
4.	Regarder le Verifiable Secret Sharing (+recovery ?)[1,2], qui permet de faire du secret sharing en présence de writer Byzantin.
5.	Implémentation de la solution (avec Zenoh), Évaluation des performances .
6.	Dans la solution [1], la limite tau<= n-2f, comprendre la limitation
    7.	Formaliser une propriété d’Eventual Completeness (et étudier les conséquences sur les différent threshold)
    8.	Étudier aussi l’auditability avec d’autre type de faute: only crash, en autorisant les Byzantins à coopérer, et en considérant les Byzantins comme un adversaire unique (formaliser l’auditability dans ce cas).


==> algorithms/asynchronousCase/auditClientAsyncUnbound.tex <==
\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]

\Statex Initialization
\Statex $ ts \gets 0$ \label{line:async:unboundStrong:initTs}
\Statex $ b_i \gets \perp\, \forall i  \in [1,n]$
\Statex $ \writerAcks[i] \gets \perp,\, \forall i  \in [1,n]$

\Statex


\START[Write]($v$)\{
\State{$ts \gets ts+1$} \label{line:async:unboundStrong:incts}
\State{$[b_1,\ldots,b_n]\gets \generatesBlock(v) $} 
\START[\texttt{broadcast}]$(\writets,ts,[b_1,\ldots,b_n])$ to all servers
\label{line:async:unboundStrong:writeTs}
\EndPhase
\State{\textbf{wait until} $|\{x:\writerAcks[x]= ts\}|\geq n-f$}
\label{line:async:unboundStrong:writeTsWaitAck}

\State{\textbf{return}}
\EndPhase
\Statex \}
\Statex

\START[upon \texttt{receive}] ($\writetsack,t$) from server $\ps{i}$
\START[if] ($ts=t$) \,\{ $\writerAcks[i]\gets t$\}
\EndPhase
\EndPhase

\Statex

\START[Audit()]\{
\Statex $\collectedLog[i] \gets \emptyset, \forall i \in [1,n] $
\START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\AuditReq)$ to server $\ps{i}$
\label{line:async:unboundStrong:auditRequest}
\EndPhase
\State \textbf{wait until} $ |\{i:\collectedLog[i]\not=\emptyset\}|\geq n-f$
\label{line:async:unboundStrong:waitAuditResponse}
\START[for] \textbf{all}$(\pr,ts,\nSeq)\in \bigcup_{i\in[1,n]}\collectedLog[i]$ %\textbf{do}
% \START[for] \textbf{all} $(\pr,v,wsn,rsn)$ with wsn the greatest sequence number
\START[for] $1\leq k\leq n$  \textbf{if} $(\pr,ts,\nSeq)_{\sigma_{\pr}} \in \collectedLog[k]$  $\land(\pr,ts,\nSeq)_{\sigma_{\pr}}\not \in E_A$
\State\textbf{then} $E_A\gets E_A\cup (\pr,ts,\nSeq)_{\sigma_{\pr}}$
\EndPhase
% \textbf{then} $\mathcal{E}_{\pr,ts,\nSeq}\gets\mathcal{E}_{\pr,ts,\nSeq}\cup\{k\} $
% \State{\textbf{if} $|\mathcal{E}_{\pr,ts,\nSeq}|\geq =t$ \textbf{then} $E_A\gets E_A\cup (\pr,ts,\nSeq)_{\sigma_{\pr}} $}
\label{line:async:unboundStrong:conditionReportAudit}
% \EndPhase
\EndPhase
\State{\textbf{return} $E_A$} 
% \Comment{For the accountability use sign message}

\EndPhase
\Statex \}

\START[upon \texttt{receive}] ($\AuditResp, \Logi$) from server $\ps{i}$
\State \textbf{if} $\Logi=\emptyset$ \textbf{then} \{ $\collectedLog[i]\gets \perp$ \}
\State \textbf{else} $\collectedLog[i]\gets \Logi$
\EndPhase

\end{algorithmic}
}
    \caption{Pseudo-code of the write and audit operations at writer $\pw$.}
    \label{alg:async:unboundStrong:AtomicRegisterClientWrite}
\end{figure}




\begin{figure}[!htpb]
{\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Definitions:}
% \Statex $\ValidBlock( \langle ts\rangle) \triangleq \{v|\exists \{b\}\in Values[ts], \GetBlock(\{b\})=v\}\land valid(v)$ 
\Statex $\ValidBlock(ts) \triangleq  {\sf \GetValue} (\collectedValues)=(v,ts)$ 
% \Statex $\notOld(ts) \triangleq |\{i:max(\collectedTs[i])\leq ts\}|\geq 2f+1$
\Statex \textcolor{black}{ $\notOld( ts) \triangleq |\{i:min(\collectedTs[i])\leq ts\}|\geq 2f+1$ }
\Statex


\Statex \textbf{Initialization :}
\Statex $\nSeq \gets 0$
\Statex $\collectedValues[i] \gets (\perp,\perp), \forall i \in [1,n] $
\Statex $\collectedTs[i] \gets \emptyset, \forall i \in [1,n] $
\Statex $\smallestTimestamp \gets \perp$
\Statex
\START[Read()]\{
\State{$\nSeq \gets \nSeq+1$}
\State $\collectedValues[i] \gets (\perp,\perp), \forall i \in [1,n] $
\State $\collectedTs[i] \gets \emptyset, \forall i \in [1,n] $
% \State $\fwd[i] \gets \perp, \forall i \in [1,n]$
\State $\smallestTimestamp \gets \perp$

% \START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\getts,\nSeq)$ to server $\ps{i}$
% \EndPhase
\START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\getts,\nSeq)$ to server $\ps{i}$
\label{line:async:unboundStrong:sendGetTs}

\EndPhase
\State \textbf{wait until}
$(|\{ts\in\collectedTs:ts=\smallestTimestamp\}|\geq f+1)$
\label{line:async:unboundStrong:conditionGetBlock}

% \START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\GetBlocks,(\pr,\smallestTimestamp,\nSeq)_{\sigma(\pr)})$ \Statex 
% \hfill to server $\ps{i}$
% \EndPhase
\START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\GetBlocks,(\pr,\smallestTimestamp,\nSeq)_{\sigma_{\pr}})$ to server $\ps{i}$
\label{line:async:unboundStrong:sendGetBlocks}
\EndPhase

\State \textbf{wait until}
$(\ValidBlock(ts)\land\notOld(ts))$
\label{line:async:unboundStrong:conditionread}

\label{line:async:unboundStrong:endReadMessage}
\State \textbf{return}  $\GetValue(\collectedValues)$
\label{line:async:unboundStrong:readReturn}

\EndPhase
\Statex
\Statex

\START[upon \texttt{receive}]{ (\TS,ts,num) from server $\ps{i}$}
\START[if] ($num=\nSeq$)
    \State $\collectedTs[i]\gets \collectedTs[i]\cup ts$
    \label{line:async:unboundStrong:tsRepColectTs}
    \START[if] $(|x:\collectedTs[x]\not=\perp\}|\geq n-f$
    \State\textcolor{black}{ $\smallestTimestamp \gets min(\{ts\in \collectedTs$ $|$ $\notOld(ts)\})$}
    \label{line:async:unboundStrong:notOld}
    % \START[for] { $i \in [1,n]$
    % \texttt{\textbf{send}} $(\GetValUnbound,\smallestTimestamp$, \Statex \hfill $\nSeq)$ to server $\ps{i}$}
    % \EndPhase
    \START[for] $i \in  [1,n]$ \texttt{\textbf{send}} $(\GetValUnbound,\smallestTimestamp,\nSeq)$ to server $\ps{i}$
    \label{line:async:unboundStrong:sendGetVal}
    \EndPhase
    
    % \State \texttt{\textbf{send}} $(\GetValUnbound,\smallestTimestamp,\nSeq)$ to all servers
    % \label{line:async:unboundStrong:sendGetVal}
    \EndPhase
    \EndPhase
\EndPhase

\Statex

\START[upon \texttt{receive}] ($\SendValUnbound,ts,num$) from server $\ps{i}$
\START[if] ($num=\nSeq$)
\{$\collectedTs[i]\gets \collectedTs[i]\cup ts$\}
\label{line:async:unboundStrong:valRepColectTs}
    \EndPhase
\EndPhase
\Statex

\START[upon \texttt{receive}]{ ($\SendBlock,b_{i},ts,num$) from server $\ps{i}$}
\START[if] ($num=\nSeq$)
    % \State $\fwd[i]\gets (b_{i},ts)$
    \State $\collectedValues[i]\gets (b_i,ts)$
    \label{line:async:unboundStrong:ColectBlock}
    \EndPhase
\EndPhase



% \START[Read()]\{
% \Statex $\collectedTs[i] \gets \perp, \forall i \in [1,n] $
% \Statex $\collectedValues[i] \gets \emptyset, \forall i \in [1,n] $
% % \Statex $\forall i,\, \fwd[i] \gets \emptyset$
% \Statex $\smallestTimestamp \gets \perp$
% \Statex $\writtenBackVal \gets \langle \perp,\perp\rangle$
% % \Statex $phase \gets \perp$
% % \Statex $wb2cnt \gets 0$

% \Statex

% \Statex // Phase R1
% \START[for] $i \in  [1,n]$ $send(\getts)$ to server $\ps{i}$
% \label{line:async:unboundStrong:sendGetTs}
% \EndPhase
% \START[repeat]
% \State // Wait responses

% \START[upon \texttt{receive}]{ (\TS,$\ps{i}$,ts) from server $\ps{i}$}
% \State $\collectedTs[i]\gets ts$
% \EndPhase
% % \START[upon \texttt{receive}]{ (\FWD,$\Vals_{i}$,ts) from server $\ps{i}$}
% % \State $\fwd[i]\gets \Vals_{i}$
% % \State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
% % \EndPhase
% % \State{// Wait responses}
% \EndPhase
% \State \textbf{until} $(|x:\collectedTs[x]\not=\perp\}|\geq n-f$
% \label{line:async:unboundStrong:endPhaseR1}
% \Statex

% \Statex // Phase R2
% % \State $\phase \gets R2$
% \State{ $\smallestTimestamp \gets min(\{ts\in \collectedTs$ $|$ $\notOld(ts)\land \isSigned(ts)\})$}
% % \Comment{There is no write operation that terminates for a timestamp $t'>\smallestTimestamp$.}
% \START[for] $i \in  [1,n]$ $send(\getval,\smallestTimestamp,\textcolor{red}{\signMessage{\pr,\smallestTimestamp}{\pr}})$ to server $\ps{i}$
% \EndPhase

% % \State{$\smallestTimestamp \gets min(\{ts|\notOld(ts)==true\})$}
% % \START[for] $i \in  [1,n]$ $send(\getval,\smallestTimestamp)$ to server $i$
% \START[repeat]
% \State // Wait responses

% % \START[if]{$|\{\ps{i}, \collectedValues[i].ts=ts\}|\geq f+1$}
% % \START[for] $i \in  [1,n]$ send($\wbackval$,ts,$\collectedTsShare)$ to server $\ps{i}$
% % \label{line:async:unboundStrong:writeBack1}
% % \EndPhase
% % \EndPhase
% % \START[upon \texttt{receive}]{ ($\FWD,\Vals_{i},ts$) from server $\ps{i}$}
% % \State $\fwd[i]\gets \Vals_{i}$
% % \State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
% % \EndPhase

% \Statex
% \START[upon \texttt{receive}]{ (\TS,$\ps{i}$,ts) from server $\ps{i}$}
% % \START[if] {$\phase=R2\lor\phase=R1$}
% \State $\collectedTs[i]\gets ts$
% % \EndPhase
% % \START[if] {$\phase=R2$}
% \State{\tiny $\smallestTimestamp \gets min(\{ts\in \collectedTs$ $|$ $\notOld(ts)=true\langle \isSigned(ts,\pw)\})$} \label{line:async:unboundStrong:notOld}
% % \Comment{There is no write operation that terminates for a timestamp $t'>\smallestTimestamp$.}
% \START[for] $i \in [1,n]$ $send(\GetValUnbound,\smallestTimestamp,\textcolor{red}{\signMessage{\pr,\smallestTimestamp}{\pr}})$ to server $\ps{i}$
% \label{line:async:unboundStrong:sendGetVal}
% \EndPhase
% \EndPhase
% % \EndPhase

% \Statex

% \START[upon \texttt{receive}]($\SendValUnbound$,$\Vals_{i},\shareVal$) from server $\ps{i}$
% % \START[if] {$\phase=R2$}
% \State $\collectedValues[i]\gets \collectedValues[i]\cup \Vals_{i}$
% % \State $\collectedValShare[s]\gets \shareVal$
% % \State $\collectedShares_r[s]\gets \collectedShares_r[s]\cup \Vals.share$
% \EndPhase
% % \EndPhase
% % \State // Wait responses
% \EndPhase
% \State \textbf{until}
% $(|ts:\collectedTs bis[i]=ts|\geq f+1)\land (\notOld(\langle ts\rangle))$
% \label{line:async:unboundStrong:conditionread}
% % \Statex // Phase Wb2
% % \State{$phase \gets WB2$}
% \Statex // Phase R3
% \textcolor{red}{
% \START[for] $i \in  [1,n]$ $send(\GetSignature,ts,BLS)$ to server $\ps{i}$
% % \EndPhase
% }
% \label{line:async:unboundStrong:BLSReadMessage}
% \START[repeat]
% \State // Wait responses
% \EndPhase
% \State \textbf{until} $ 2f+1 responses.$

% \Statex // Phase R4
% \textcolor{red}{
% \START[for] $i \in  [1,n]$ $send(\GetBlocks,ts,BLS)$ to server $\ps{i}$
% % \EndPhase
% }
% \label{line:async:unboundStrong:BLSReadMessage}
% \START[repeat]
% \State // Wait responses
% \EndPhase
% \State \textbf{until} $ 2f+1 responses.$
% \State $\writtenBackVal \gets \GetValue( \langle ts,\collectedValues \rangle)$

% % \EndPhase
% % \START[repeat]
% % \State{// Wait responses}
% % \EndPhase
% % \State \textbf{until} (receives n-f $\wbacktsack$ messages)
% % \label{line:async:unboundStrong:waitWritebackTsAck}
% \State \textbf{return} $\writtenBackVal$
% \label{line:async:unboundStrong:readReturn}

% \EndPhase
% \Statex \}
% \Statex


\end{algorithmic}
}
\caption{Pseudo-code of the read operation at reader $\pr$.}
\label{alg:async:unboundStrong:AtomicRegisterClientRead}
\end{figure}




% \begin{figure}[!htpb]
% {\footnotesize
% \begin{algorithmic}[1]

% \Statex

% \START[Audit()]\{
% \Statex $\collectedLog[i] \gets \emptyset, \forall i \in [1,n] $
% \START[for] $i \in  [1,n]$ \texttt{\textbf{send}}$(\AuditReq)$ to server $\ps{i}$
% \label{line:async:unboundStrong:auditRequest}
% \EndPhase
% \State \textbf{wait until} $ |\{i:\collectedLog[i]\not=\emptyset\}|\geq n-f$
% \label{line:async:unboundStrong:waitAuditResponse}
% \START[for] \textbf{all}$(\pr,ts,\nSeq)\in \bigcup_{i\in[1,n]}\collectedLog[i]$ %\textbf{do}
% % \START[for] \textbf{all} $(\pr,v,wsn,rsn)$ with wsn the greatest sequence number
% \START[for] $1\leq k\leq n$  \textbf{if} $(\pr,ts,\nSeq)_{\sigma_{\pr}} \in \collectedLog[k]$
% \Statex \hfill $\land(\pr,ts,\nSeq)_{\sigma_{\pr}}\not \in E_A$
% \State\textbf{then} $E_A\gets E_A\cup (\pr,ts,\nSeq)_{\sigma_{\pr}}$
% \EndPhase
% % \textbf{then} $\mathcal{E}_{\pr,ts,\nSeq}\gets\mathcal{E}_{\pr,ts,\nSeq}\cup\{k\} $
% % \State{\textbf{if} $|\mathcal{E}_{\pr,ts,\nSeq}|\geq =t$ \textbf{then} $E_A\gets E_A\cup (\pr,ts,\nSeq)_{\sigma_{\pr}} $}
% \label{line:async:unboundStrong:conditionReportAudit}
% % \EndPhase
% \EndPhase
% \State{\textbf{return} $E_A$} 
% % \Comment{For the accountability use sign message}

% \EndPhase
% \Statex \}

% \START[upon \texttt{receive}] ($\AuditResp, \Logi$) from server $\ps{i}$
% \State \textbf{if} $\Logi=\emptyset$ \textbf{then} \{ $\collectedLog[i]\gets \perp$ \}
% \State \textbf{else} $\collectedLog[i]\gets \Logi$
% \EndPhase

% \end{algorithmic}
% }
% \caption{Audit operation of \algAsyncRBSign\, solution.}
% \label{alg:async:unboundStrong:AtomicRegisterClientAudit}
% \end{figure}






==> algorithms/asynchronousCase/auditServerAsyncUnbound.tex <==
\begin{figure}[!htpb]
{
\footnotesize
\begin{algorithmic}[1]
\Statex Initialization
\Statex $\Rts_{i} \gets  0$
\Statex $\RVal_{i} \gets \emptyset$
% \Statex $\RValblock \gets \emptyset$
\Statex $\Logi \gets \emptyset$
\Statex $\READERS_{i} \gets \emptyset$
\Statex $\READERS_{i} \gets \emptyset$
\Statex $\writerAcks_{i}[i] \gets \{\emptyset\}, \forall i \in [1,n]$

\label{line:async:unboundStrong:init}

\Statex

\Statex // Write Protocol Messages
\Comment{Pseudo code for server i}

% \Statex 
\START[upon \texttt{receive}] ($\writets,ts,[b_1,\ldots,b_n]$) from writer $\pw$
\label{line:async:unboundStrong:receiveWriteVal}
\State $\RVal_{i} \gets \RVal_{i} \cup (b_{i},ts)$
\label{line:async:unboundStrong:updateRValWriteVal}
% \State $\Blocks_{i} \gets \RVal_{i} \cup (b_{i},ts)$
% \label{line:async:unboundStrong:updateBlocksWriteVal}
\START[if] {$\Rts_{i}<ts$}
\{$\Rts_{i} \gets ts$\}
\label{line:async:unboundStrong:updateRts}
\EndPhase
\State \texttt{\textbf{send}} $\writetsack$ to $\pw$
\label{line:async:unboundStrong:writeAck}
\EndPhase
% \Statex

% \START[on receive] ($\getReaders$,ts) from reader $\pr$ 
% \State send($\sendReaders$,$\READERS_{i}$,ts) to $\pr$
% \label{line:async:unboundStrong:concurrentReaderServer}
% \EndPhase

\Statex

\Statex // Read Protocol Messages
\START[upon \texttt{receive}] ($\getts,\nSeq$) from reader $\pr$
\State{\texttt{\textbf{send}}($\TS,\Rts,\nSeq)$)}
\label{line:async:unboundStrong:sendTs}
\EndPhase

\Statex 

\START[upon \texttt{receive}] ($\GetValUnbound,ts,\nSeq $) from reader $\pr$
% \START \textcolor{red}{($\checkSignature(ts,\pw) = true$)}
\START[wait for] ($\Rts \geq ts )$
\label{line:async:unboundStrong:waitTsSendTs}
\State \texttt{\textbf{send}}($\SendValUnbound,ts,\nSeq$) to $\pr$
\label{line:async:unboundStrong:sendTs2}
\EndPhase
\EndPhase





\Statex

% \START[on receive] $(\GetSignature,ts)$ from reader $\pr$ \label{line:async:receiveGetSignature}
% \START \textcolor{red}{($\checkSignature(ts,f+1) = true$)}
% \State $\Logi \gets \Logi\cup \langle \pr,ts,\textcolor{red}{\sigma_{\pr}(\pr,ts)} \rangle$
% \label{line:async:unboundStrong:logServRval}
% \State send($\GetSignatureAck,\signMessage{ts,\pr}{\ps{i}}$) to $\pr$
% \EndPhase
% \EndPhase

\START[upon \texttt{receive}] $(\GetBlocks,(\pr,ts,\nSeq)_{\sigma(\pr)})$ from reader $\pr$
\label{line:async:unboundStrong:receiveGetBlocks}
% \START \textcolor{red}{($\checkSignature(ts,2f+1) = true$)}
\START[wait for] $\Rts\geq ts$
\label{line:async:unboundStrong:waitTsSendVal}
\State \texttt{\textbf{broadcast}}($Valid\_Req,ts,\nSeq$) to all servers
\label{line:async:unboundStrong:sendValidReq}
\State{\textbf{wait until} $|\{x:\writerAcks[x][\nSeq]= ts\}|\geq n-f$}
\label{line:async:unboundStrong:waitValidResp}
\State $\Logi \gets \Logi \cup
(\pr,ts,\nSeq)_{\sigma(\pr)}$
\label{line:async:unboundStrong:logServRval}
\State \texttt{\textbf{send}}($\SendBlock,\RVal[ts],\nSeq$) to $\pr$
\label{line:async:unboundStrong:sendVal}
\EndPhase
\EndPhase

\Statex

\START[upon \texttt{receive}] ($Valid\_Req,ts,\nSeq $) from server $\ps{j}$
% \START \textcolor{red}{($\checkSignature(ts,\pw) = true$)}
\START[wait for] ($\Rts \geq ts )$
\label{line:async:unboundStrong:waitTsValidReq}
\State \texttt{\textbf{broadcast}}($Valid\_Resp,ts,\nSeq$) to all servers
\label{line:async:unboundStrong:sendValidResp}
\EndPhase
\EndPhase

\Statex

\START[upon \texttt{receive}] ($Valid\_Resp,ts,\nSeq $) from server $\ps{j}$
\State $\writerAcks[j][\nSeq]= ts$
\label{line:async:unboundStrong:receiveValidResp}
\EndPhase

\Statex

\Statex // Audit protocol Messages
\START[upon \texttt{receive}] ($\AuditReq$) from owner $\pR$ of R 
\State \texttt{\textbf{send}}($\AuditResp$,$\Logi$) to $\pR$
\label{line:async:unboundStrong:senLog}
% \State $\Log \gets \emptyset$
% \Comment{Audit operation is performed by correct and detect operation between two audit operation, be careful to not lose any information with concurrent read operation}

\EndPhase
\Statex

\end{algorithmic}{}
}
\caption{Pseudo-code at server $\ps{i}$.}
\label{alg:async:unboundStrong:AtomicRegisterServer}
\end{figure}{}



==> conclusion.tex <==
% This paper investigated the problem of implementing an auditable register in a Byzantine setting. 
% We formally proved that, as suggested in \cite{CB20}, without communication between servers, auditability requires $4f+1$ servers. Our impossibility is proved for a safe register, which provides the weakest semantic in the Lamport's hierarchy \cite{L86}. Our impossibility result implies that the solution provided by \cite{CB20}, is optimal resilient in that setting. On the other hand, allowing servers to communicate with each other, we present an algorithm that implements an auditable atomic register which requires only $3f+1$ servers. Our algorithm is optimal resilient, because there is a well known result that proves that $3f+1$ servers are necessary to implement an atomic register if at most $f$ servers can be Byzantine\cite{MAD02}.

% Our algorithm guarantees that if a client never read the register it is never detected, and any client that read a value is detected for that value. However, our algorithm is not perfectly accurate in the sense that a client that read a value could be additionally detected to have read a value that it never read. It could be interesting to consider if a stronger accuracy property can be implemented together with atomicity and which complexity cost (local space, number of servers and message complexity). Interestingly, having strong accuracy is a first step toward accountability \cite{peerreview}, that is, processes cannot repudiate their actions.


==> diagram/impossibilityConsensus3process.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,396); %set diagram left start at 0, and has height of 396

%Rounded Rect [id:dp17224174912773804] 
\draw   (199.81,38.13) .. controls (199.81,33.82) and (203.3,30.33) .. (207.61,30.33) -- (242.21,30.33) .. controls (246.51,30.33) and (250,33.82) .. (250,38.13) -- (250,61.51) .. controls (250,65.81) and (246.51,69.3) .. (242.21,69.3) -- (207.61,69.3) .. controls (203.3,69.3) and (199.81,65.81) .. (199.81,61.51) -- cycle ;

%Rounded Rect [id:dp46832748632373833] 
\draw   (199.81,138.31) .. controls (199.81,134.01) and (203.3,130.52) .. (207.61,130.52) -- (242.21,130.52) .. controls (246.51,130.52) and (250,134.01) .. (250,138.31) -- (250,161.69) .. controls (250,165.99) and (246.51,169.48) .. (242.21,169.48) -- (207.61,169.48) .. controls (203.3,169.48) and (199.81,165.99) .. (199.81,161.69) -- cycle ;

%Rounded Rect [id:dp39172595928071285] 
\draw   (325.22,138.31) .. controls (325.22,134.01) and (328.71,130.52) .. (333.01,130.52) -- (367.61,130.52) .. controls (371.92,130.52) and (375.41,134.01) .. (375.41,138.31) -- (375.41,161.69) .. controls (375.41,165.99) and (371.92,169.48) .. (367.61,169.48) -- (333.01,169.48) .. controls (328.71,169.48) and (325.22,165.99) .. (325.22,161.69) -- cycle ;

%Rounded Rect [id:dp3085904817470828] 
\draw   (74.68,138.31) .. controls (74.68,134.01) and (78.17,130.52) .. (82.48,130.52) -- (117.08,130.52) .. controls (121.38,130.52) and (124.87,134.01) .. (124.87,138.31) -- (124.87,161.69) .. controls (124.87,165.99) and (121.38,169.48) .. (117.08,169.48) -- (82.48,169.48) .. controls (78.17,169.48) and (74.68,165.99) .. (74.68,161.69) -- cycle ;

%Rounded Rect [id:dp8951579314714962] 
\draw   (116.41,338.82) .. controls (116.41,334.51) and (119.9,331.03) .. (124.2,331.03) -- (158.8,331.03) .. controls (163.1,331.03) and (166.59,334.51) .. (166.59,338.82) -- (166.59,362.2) .. controls (166.59,366.5) and (163.1,369.99) .. (158.8,369.99) -- (124.2,369.99) .. controls (119.9,369.99) and (116.41,366.5) .. (116.41,362.2) -- cycle ;

%Rounded Rect [id:dp05004686960801674] 
\draw   (33.43,338.82) .. controls (33.43,334.51) and (36.92,331.03) .. (41.23,331.03) -- (75.83,331.03) .. controls (80.13,331.03) and (83.62,334.51) .. (83.62,338.82) -- (83.62,362.2) .. controls (83.62,366.5) and (80.13,369.99) .. (75.83,369.99) -- (41.23,369.99) .. controls (36.92,369.99) and (33.43,366.5) .. (33.43,362.2) -- cycle ;

%Rounded Rect [id:dp3508164062420115] 
\draw   (325.22,238.81) .. controls (325.22,234.51) and (328.71,231.02) .. (333.01,231.02) -- (367.61,231.02) .. controls (371.92,231.02) and (375.41,234.51) .. (375.41,238.81) -- (375.41,262.19) .. controls (375.41,266.49) and (371.92,269.98) .. (367.61,269.98) -- (333.01,269.98) .. controls (328.71,269.98) and (325.22,266.49) .. (325.22,262.19) -- cycle ;

%Rounded Rect [id:dp5522394188335493] 
\draw   (199.81,238.81) .. controls (199.81,234.51) and (203.3,231.02) .. (207.61,231.02) -- (242.21,231.02) .. controls (246.51,231.02) and (250,234.51) .. (250,238.81) -- (250,262.19) .. controls (250,266.49) and (246.51,269.98) .. (242.21,269.98) -- (207.61,269.98) .. controls (203.3,269.98) and (199.81,266.49) .. (199.81,262.19) -- cycle ;

%Rounded Rect [id:dp11667403080611827] 
\draw   (116.41,238.81) .. controls (116.41,234.51) and (119.9,231.02) .. (124.2,231.02) -- (158.8,231.02) .. controls (163.1,231.02) and (166.59,234.51) .. (166.59,238.81) -- (166.59,262.19) .. controls (166.59,266.49) and (163.1,269.98) .. (158.8,269.98) -- (124.2,269.98) .. controls (119.9,269.98) and (116.41,266.49) .. (116.41,262.19) -- cycle ;

%Rounded Rect [id:dp18420960768199846] 
\draw   (33.43,238.81) .. controls (33.43,234.51) and (36.92,231.02) .. (41.23,231.02) -- (75.83,231.02) .. controls (80.13,231.02) and (83.62,234.51) .. (83.62,238.81) -- (83.62,262.19) .. controls (83.62,266.49) and (80.13,269.98) .. (75.83,269.98) -- (41.23,269.98) .. controls (36.92,269.98) and (33.43,266.49) .. (33.43,262.19) -- cycle ;

%Straight Lines [id:da991715516641552] 
\draw    (199.81,61.51) -- (118.61,129.24) ;
\draw [shift={(117.08,130.52)}, rotate = 320.17] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5202581192660125] 
\draw    (250,61.51) -- (331.47,129.24) ;
\draw [shift={(333.01,130.52)}, rotate = 219.74] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da19067567479484615] 
\draw    (224.91,68.82) -- (224.91,128.52) ;
\draw [shift={(224.91,130.52)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da05790752144073008] 
\draw    (99.78,169.48) -- (123.46,229.16) ;
\draw [shift={(124.2,231.02)}, rotate = 248.35] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2271029363720093] 
\draw    (99.78,169.48) -- (76.55,229.15) ;
\draw [shift={(75.83,231.02)}, rotate = 291.27] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8341572985325397] 
\draw    (58.53,269.98) -- (58.53,329.03) ;
\draw [shift={(58.53,331.03)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5773101484763193] 
\draw    (141.5,269.98) -- (141.5,329.03) ;
\draw [shift={(141.5,331.03)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9207714074742316] 
\draw    (224.91,169.48) -- (224.91,229.02) ;
\draw [shift={(224.91,231.02)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8562244525934176] 
\draw    (350.31,169.48) -- (350.31,229.02) ;
\draw [shift={(350.31,231.02)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (219.41,41.32) node [anchor=north west][inner sep=0.75pt]   [align=left] {s};
% Text Node
\draw (219.41,141.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$s_{B}$};
% Text Node
\draw (344.81,141.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$s_{C}$};
% Text Node
\draw (94.28,141.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {};
% Text Node
\draw (136,342.01) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (53.03,342.01) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (344.81,242) node [anchor=north west][inner sep=0.75pt]   [align=left] {0};
% Text Node
\draw (219.41,242) node [anchor=north west][inner sep=0.75pt]   [align=left] {0};
% Text Node
\draw (136,242) node [anchor=north west][inner sep=0.75pt]   [align=left] {$s'_{C}$};
% Text Node
\draw (53.03,242) node [anchor=north west][inner sep=0.75pt]   [align=left] {$s'_{B}$};
% Text Node
\draw (75.78,79.82) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {A reads \\a register};
% Text Node
\draw (226.91,172.48) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize B runs}\\{\scriptsize solo}};
% Text Node
\draw (352.31,172.48) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize C runs}\\{\scriptsize solo}};
% Text Node
\draw (143.5,272.98) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize C runs}\\{\scriptsize solo}};
% Text Node
\draw (60.53,272.98) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize B runs}\\{\scriptsize solo}};
% Text Node
\draw (121.5,173.48) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize C executes}\\{\scriptsize  one operation}};
% Text Node
\draw (314.81,72.82) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize C executes}\\{\scriptsize  one operation}};
% Text Node
\draw (14.53,173.48) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize B executes}\\{\scriptsize  one operation}};
% Text Node
\draw (227.91,89.82) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize B executes}\\{\scriptsize  one operation}};


\end{tikzpicture}


==> diagram/tableConsensusrTwoProcess.tex <==
\begin{table}[!h]
        \centering
        
\begin{tabular}{|p{0.32\textwidth}|p{0.10\textwidth}|p{0.10\textwidth}|p{0.14\textwidth}|p{0.09\textwidth}|p{0.09\textwidth}|p{0.16\textwidth}|}
\hline 
 Scenario & p\textsubscript{1} read & p\textsubscript{1} audit & p\textsubscript{1} return & p\textsubscript{0} read & p\textsubscript{0} audit & p\textsubscript{0} return \\
\hline 
 123456 & v\textsubscript{0} & (p\textsubscript{0},丄) & v\textsubscript{0} & 丄 & 丄 & v\textsubscript{0} \\
\hline 
 124536 (124563)  & v\textsubscript{0} & (p\textsubscript{0},丄) & v\textsubscript{0} & 丄 & (p\textsubscript{1},v\textsubscript{0}) & v\textsubscript{0} \\
\hline 
 \makecell[l]{142536 (142563) (145263) (145236)\\412536 (412563) (415263) (415236)} & v\textsubscript{0} & (p\textsubscript{0},v\textsubscript{1}) & v\textsubscript{1} & v\textsubscript{1} & (p\textsubscript{1},v\textsubscript{0}) & v\textsubscript{1} \\
\hline 
 145623 (415623) & v\textsubscript{0} & 丄 & v\textsubscript{1} & v\textsubscript{1} & (p\textsubscript{1},v\textsubscript{0}) & v\textsubscript{1} \\
\hline 
 142356 (412356) & v\textsubscript{0} & (p\textsubscript{0},v\textsubscript{1}) & v\textsubscript{1} & v\textsubscript{1} & 丄 & v\textsubscript{1} \\
\hline 
 451263 (451236) & 丄 & (p\textsubscript{0},v\textsubscript{1}) & v\textsubscript{1} & v\textsubscript{1} & (p\textsubscript{1},丄) & v\textsubscript{1} \\
\hline 
 456123 & 丄  & 丄 & v\textsubscript{1} & v\textsubscript{1} & (p\textsubscript{1},丄) & v\textsubscript{1} \\
 \hline
\end{tabular}
        
        \end{table}

==> proof/atomicityUnbound.tex <==


According to line \ref{line:async:unbound:updateRts} figure \ref{alg:async:unbound:AtomicRegisterServer}
% \ref{line:async:unbound:writetsRts} figure \ref{alg:async:unbound:AtomicRegisterServer}
the following observation holds :

\begin{observation}
\label{observation:unbound:tsMonotonicallyIncrease}
A correct server $\ps{i}$ updates $\Rts$ with a new timestamp, only if this timestamp is greater than the previous one stored in $\Rts$. Hence, timestamps stored at correct servers increase monotonically
\end{observation}

\noindent{}
\begin{lemma}
\label{lemma:async:unbound:writerEndWriteServerTimestamp}
Let $\op{w}$ be a write operation with timestamp $ts$. After $\op{w}$ returns the value of $\Rts$ is greater than or equal to $ts$ in at least $f+1$ correct servers. 

\end{lemma}\spaceLemmaProof 

\begin{proofL}
$\op{w}$ terminates when the condition at line \ref{line:async:unbound:writeTsWaitAck} of figure \ref{alg:async:unbound:AtomicRegisterClientWrite} is evaluated to true. 
Hence, $\op{w}$ terminates only if the writer received  $(\writetsack,ts)$, from at least $2f+1$ different servers. 
A correct server, sends $(\writetsack,ts)$ (line \ref{line:async:unbound:writeAck} of figure \ref{alg:async:unbound:AtomicRegisterServer}) to the writer, if it receives $(\writets,ts,-,-,-)$ from the writer and after the execution of line \ref{line:async:unbound:updateRts} in Figure \ref{alg:async:unbound:AtomicRegisterServer}
Since there are at most $f$ of the $3f+1$ servers are Byzantine, once the write operation completes, the writer has received at least $f+1$  $(\writetsack,ts)$ from correct servers.
Observation \ref{observation:unbound:tsMonotonicallyIncrease} concludes the proof. 

\renewcommand{\toto}{lemma:async:unbound:writerEndWriteServerTimestamp}
\end{proofL}



\begin{lemma}
\label{lemma:async:unbound:readerEndWriteServerTimestamp}
Let $\op{r}$ be a complete read operation and let $ts$ the timestamp corresponding to the value it returns. At any time after $\op{r}$ returns the value of $\Rts$ is greater than or equal to $ts$ in at least $f+1$ correct servers. 
\end{lemma}\spaceLemmaProof 


\begin{proofL}
Since $\op{r}$ terminates, it has satisfied the condition $\ValidBlock(ts)$ (line \ref{line:async:unbound:conditionread} figure \ref{alg:async:unbound:AtomicRegisterClientRead}). For this condition to be true, the reader must have received $2f+1$ different valid blocks for timestamp $ts$, piggybacked by $\VALS$ messages (lines \ref{line:async:unbound:valRepColectTs} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) sent by different servers. A correct server sends such messages, only after it has $\Rts\geq ts$ (lines \ref{line:async:unbound:waitTsSendVal} and \ref{line:async:unbound:updateRts}).
Since there are at most $f$ Byzantine servers, and by observation \ref{observation:unbound:tsMonotonicallyIncrease}, the claims follow.

\renewcommand{\toto}{lemma:async:unbound:readerEndWriteServerTimestamp}
\end{proofL}


\begin{lemma}
\label{lemma:async:unbound:W-Ratomicity}
Let $\op{w}$ be a complete write operation with timestamp $ts$ and let $\op{r}$ be a complete read operation by a correct process $\pr$ associated to a timestamp $ts'$. If $\op{r}$ succeeds $\op{w}$ in real-time order then $ts' \geq ts$
\end{lemma}\spaceLemmaProof 

\begin{proofL}
Since $\op{r}$ returns a value associated to timestamp $ts'$, the condition $\notOld(ts')$ (line \ref{line:async:unbound:conditionread} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) is satisfied. 
In the following, we show that $\notOld(ts')$ true implies that $ts'\geq ts$.

Let us consider that $\notOld(ts')$ is true. 
As $\collectedTs$ is reinitialized at the beginning of each new read operation, $\notOld(ts')$ is true, if all timestamps receives from at least $2f+1$ different servers piggybacked by $\SendValUnbound$ (line \ref{line:async:unbound:valRepColectTs} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) or $\TS$ (line \ref{line:async:unbound:valRepColectTs} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) messages are smaller than or equal to $ts'$.
According to Lemma \ref{lemma:async:unbound:writerEndWriteServerTimestamp}, as $\op{w}$ terminates, the content of $\Rts$ is greater than or to equal  $ts$ in at least $f+1$ correct servers.
So, during $\op{r}$, in response to $(\getval,\nSeq)$ (line \ref{line:async:unbound:sendVal} figure \ref{alg:async:unbound:AtomicRegisterServer}), the reader can collect at most $2f=n-(n-2f)$ messages for a timestamp smaller than $ts$. Thus, $\notOld()$ always remain false for any timestamp smaller than $ts$, and since $\notOld(ts')$ is true,  $ts'\geq ts$.



\renewcommand{\toto}{lemma:async:unbound:W-Ratomicity}

\end{proofL}

\begin{lemma}
\label{lemma:async:unbound:returnWrittenValue}
If a complete read operation $\op{r}$, invoked by a correct process $\pr$,  returns a value corresponding to a timestamp $ts>0$, then it exists a write operation $\op{w}$, with timestamp $ts$, that starts before $\op{r}$ terminates.

\end{lemma}\spaceLemmaProof 
\begin{proofL}
Since $\op{r}$ terminates, it has satisfied the condition $\ValidBlock(ts)$ (line \ref{line:async:unbound:conditionread} of Figure \ref{alg:async:unbound:AtomicRegisterClientRead}). Thus, the reader received $2f+1$ distinct valid blocks for timestamp $ts$, piggybacked by $\SendBlock$  messages (lines \ref{line:async:unbound:receiveGetBlocks} and of Figure \ref{alg:async:unbound:AtomicRegisterClientRead}) sent by distinct servers. As all the variables are reinitialized at the beginning of a read operation, and as there are at most $f$ Byzantine servers, at least $f+1$  correct servers sent a block to $\pr$ during the execution of $\op{r}$. 
A correct server $\pss$ sends a block corresponding to a timestamp $ts>0$ only after it has received the corresponding $\writets$ message from the writer; thus, after the invocation of a write operation $\op{w}$ for timestamp $ts$. It follows that $\op{w}$ began before $\op{r}$ completes.

\renewcommand{\toto}{lemma:async:returnWrittenValue}
\end{proofL}


\begin{lemma} 
\label{lemma:async:unbound:R-Ratomicity}
Let $\op{r}$ be a complete read operation invoked by a correct process $\pr$, and let $\op{r'}$ be a complete read operation invoked by a correct process $\pr'$ ($\pr$ and $\pr'$ may be the same process). Let $ts$ and $ts'$ be the timestamps associated with $\op{r}$ and $\op{r'}$ respectively. If $\op{r'}$ succeeds $\op{r}$  in real-time order then $ts' \geq ts$.

\end{lemma}\spaceLemmaProof 

\begin{proofL}
The proof follows the same approach as the proof of Lemma \ref{lemma:async:unbound:W-Ratomicity}.

Let $ts'$ be $\op{r'}.ts$ and let $ts$ be $\op{r}.ts$.
As $\op{r'}$ returns a value associated to a timestamp $ts'$, the conditions $\ValidBlock(ts')$ and $\notOld(ts')$ are true for timestamp $ts$ (line \ref{line:async:unbound:conditionread} figure \ref{alg:async:unbound:AtomicRegisterClientRead}). 
In the following, we show that if condition $\notOld(ts')$ implies that $ts'\geq ts$.

Let us consider that $\notOld(ts')$ is true. 
As $\collectedTs$ is reinitialized at the beginning of each new read operation, $\notOld(ts')$ is true, if all timestamps receives from at least $2f+1$ different servers piggybacked by $\SendValUnbound$ (line \ref{line:async:unbound:valRepColectTs} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) or $\TS$ (line \ref{line:async:unbound:valRepColectTs} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) messages are smaller than or equal to $ts'$.
According to Lemma \ref{lemma:async:unbound:readerEndWriteServerTimestamp}, as $\op{r}$ returns for timestamp $ts$, then at server side, the content of $\Rts$ is greater than or to equal  $ts$ in at least $f+1$ correct servers.
So the reader can collect at most $2f=n-(n-2f)$  timestamps smaller than $ts$. Thus, $\notOld$ always remain false for any timestamp smaller than $ts$, hence $ts'\geq ts$.

\renewcommand{\toto}{lemma:async:unbound:R-Ratomicity}
\end{proofL}

\begin{lemma} 
\label{lemma:async:unbound:R-Watomicity}
Let $\op{r}$ be a complete read operation with timestamp $ts$ and let $\op{w}$ be a complete write operation by $\pw$ associated to a timestamp $ts'$. 
If $\op{w}$ succeeds $\op{r}$ in real-time order then $ts' \geq ts$
\end{lemma}\spaceLemmaProof 

\begin{proofL}
We proceed considering first the case in which $ts>0$ and then the case in which $ts=0$.
From Lemma \ref{lemma:async:unbound:returnWrittenValue}, if $ts>0$ then it exists $\op{w'}$ with timestamp $ts$ that starts before the end of $\op{r}$. Considering that, there is a unique writer and that its execution is sequential, then $\op{w'}$ terminates before $\op{w}$ starts. As timestamps growth monotonically (Observation \ref{observation:unbound:tsMonotonicallyIncrease}), 
$ts'>ts$.

Consider now the case $ts=0$. As timestamps grow monotonically (Observation \ref{observation:unbound:tsMonotonicallyIncrease}), and the initial value of the timestamp is $0$ (line \ref{line:async:unbound:initTs} of Figure \ref{alg:async:unbound:AtomicRegisterClientWrite}) then all write operations have their timestamp greater than $0$. In particular this is true for $\op{w}$, such that $ts'>ts$, which concludes the proof.
\renewcommand{\toto}{lemma:async:unbound:R-Watomicity}
\end{proofL}


% \begin{lemma}
% \label{lemma:async:unbound:Safety}
% If a read operation $\op{r}$, invoked by a correct process $\pr$ and not concurrent to any write operation, returns a value $v$, then $v$ is the value of the most recently preceding write. If there is none, $v$ is the initial value $\vo$.

% \end{lemma}\spaceLemmaProof 

% \begin{proofL}
% First we consider the cases where there is no preceding write operation, and then the case where there is one.

% Let us show by contradiction that, when there is no preceding write operation to $\op{r}$, it is impossible that $\op{r}$ returns for $v'\neq \vo$.
% In this case, as there is no write operation corresponding to $v'$, it is impossible for correct servers to send a message with a block corresponding to $v'$. However, for $\pr$  to read $v'$, the condition $\ValidBlock(ts')$ (line \ref{line:async:unbound:conditionread} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) must be satisfied. Thus, $\pr$ must  collect $2f+1$ blocks for $ts'$ from different servers in $\SendBlock$ messages. By the property of none creation of the canal of communication, $\pr$ cannot receive such messages from correct servers.Thus, $\pr$ receives those blocks from $2f+1$ Byzantine servers. As there are at most $f$ Byzantine, this is a contradiction. 

% Now, we consider the cases where a preceding write operation exists, $\op{w}$, that writes $v$ with associate timestamp $ts$. Let us show that $\op{r}$ cannot return a value $v'\neq v$. Notice that values are identifiable with their timestamp, such that $v'\neq v \Longleftrightarrow ts'\neq ts$, with $ts'$ the timestamp associate with $v'$. There are two cases to consider, (i) $ts'>ts$ and (ii) $ts'<ts$.  In case (i), $ts'>ts$, as by assumption the last write operation is $\op{w}$, and that timestamp grows monotonically (Observation \ref{observation:unbound:tsMonotonicallyIncrease}), there is no write operation  corresponding to $ts'$. Then the same arguments as before apply and gives the contradiction. In case (ii), $ts'<ts$, Lemma \ref{lemma:async:unbound:W-Ratomicity} gives the contradiction and concludes the proof.

% \renewcommand{\toto}{lemma:async:unbound:Safety}
% \end{proofL}


% \begin{theorem}
% \label{theorem:async:unbound:linearizable}
% There is a permutation $\pi$ of all completed operations in $\eventSeq$ and some subset of the pending operations such that
% if the response of operation $\op{1}$ occurs in $\eventSeq$, before the invocation of operation $\op{2}$, then $\op{1}$ appears before $\op{2}$ in $\pi$
% \end{theorem}

% \begin{proofT}
% We consider a sequence of event $\eventSeq$. In the following, we describe how to create such a permutation $\pi$ of operation. First, for each incomplete write operation $\op{w}\in\eventSeq$ associate with a value $v$, if it exists a read operation $\op{r}\in\eventSeq$ that returns $v$, then we complete $\op{w}$.

% Then, we order the operations according to their timestamp. For write operation and a read operation with the same timestamp, we order write operation before reads, and we order read operation with the same timestamp according to real time execution. Thus, from Lemma \ref{lemma:async:unbound:W-Ratomicity} and Lemma \ref{lemma:async:unbound:R-Ratomicity} if the response of an operation $\op{1}$ occurs before the invocation of an operation $\op{2}$, then $\op{1}$ appears before $\op{2}$ in $\pi$.

% \renewcommand{\toto}{theorem:async:unbound:linearizable}
% \end{proofT}





Let $E$ be any execution of our algorithm and let $H$ be the corresponding history. 
We construct ${\sf complete}(H)$ by removing all the invocations of the read operations that have no matching response and by completing a pending $write(v)$ operation if there is a complete read operation that returns $v$. Observe that only the last write operation of the writer can be pending.

Then, we explicitly construct a sequential history $\pi$ containing all the operations in ${\sf complete}(H)$. 
First we put in $\pi$ all the write operations according to the order in which they occur in $H$, because write operations are executed sequentially by the unique writer, this sequence is well-defined. Also this order is consistent with that of the timestamps associated with the values written.

Next, we add the read operations one by one, in the order of their response in $H$. A read operation that returns a value with timestamp $ts$ is placed immediately before the write that follows in $\pi$ the write operation associated to $ts$ (or at the end if this write does not exist). By construction of $\pi$ every read operation returns the value of the last preceding write in $\pi$. 
It remains to prove that $\pi$ preservers the real-time order of non-overlapping operations.
\\
\begin{theorem} \label{theorem:async:unbound:linearizable}
Let $\op{1}$ and $\op{2}$ be two operations in $H$. If $\op{1}$ ends before the invocation of $\op{2}$ then $\op{1}$ precedes $\op{2}$ in $\pi$.

\end{theorem}\spaceLemmaProof

\begin{proofT}

Since $\pi$ is consistent with the order of timestamps, we have to show that the claim is true for all operations with different timestamps.

There are four possible scenarios: 
$\op{1}$ and $\op{2}$ are respectively a write and a read operation, then the claim holds by Lemma \ref{lemma:async:unbound:W-Ratomicity}.
$\op{1}$ and $\op{2}$ are two reads operations, then the claim holds by Lemma \ref{lemma:async:unbound:R-Ratomicity}. 
$\op{1}$ and $\op{2}$ are respectively a read and a write operation, then the claim holds by Lemma \ref{lemma:async:unbound:R-Watomicity}.
If $\op{1}$ and $\op{2}$ are two write operations the claim holds by the Observation \ref{observation:unbound:tsMonotonicallyIncrease}.

\renewcommand{\toto}{theorem:async:linearizable}
\end{proofT}



==> proof/auditabilityUnbound.tex <==

\begin{lemma}
\label{lemma:async:unbound:Completeness}
Algorithm presented figure \ref{alg:async:unbound:AtomicRegisterClientWrite} to \ref{alg:async:unbound:AtomicRegisterServer} 
% with $\tau \geq 2f+1$ and $t \leq \tau-2f$ 
solves the completeness property
\end{lemma}\spaceLemmaProof 
\begin{proofL}
 For a reader $\pr$ to returns for a valid value $v$ with timestamp $ts$, then $\pr$ receives at least $\tau$ messages from different servers (line \ref{line:async:unbound:conditionread} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) with the block corresponding to $v$.
 A correct server sends a block with associate timestamp $ts$ to a reader $\pr$ (line \ref{line:async:unbound:sendVal}, figure \ref{alg:async:unbound:AtomicRegisterServer}), only after it adds to its log the reader $\pr$ associate with timestamp $ts$, line \ref{line:async:unbound:logServRval} figure \ref{alg:async:unbound:AtomicRegisterServer}. Thus, if a correct server $\pss$ sends a block with associate timestamp $ts$ to a reader $\pr$, $\pss$ stores $\pr$ ID associate with $ts$ in its log. If $\tau\geq 2f+1$, since there is at most $f$ Byzantine, in the worst case, at least $\tau-f\geq f+1$ correct servers, denoted $P_C$, records $\op{r}$ in their logs. 

Let $\op{a}$ be an audit operation, invoked by a process $\pa$, that starts after $\pr$ returns.
So when $\op{a}$ starts, $\pr$ is in PC's log. Then, $\pa$ waits $2f+1$ responses (line \ref{line:async:unbound:waitAuditResponse} figure \ref{alg:async:unbound:AtomicRegisterClientWrite}) after sending $\AUDIT$ request (line \ref{line:async:unbound:auditRequest} figure \ref{alg:async:unbound:AtomicRegisterClientWrite}) to servers. As there is at most $f$ Byzantine servers, $\pa$ gets the responses from at least $f+1$ ($n-2f$) correct servers. In particular, $\pa$ get at least one response from a server in $P_C$. Finally, with $t\leq\tau-2f=1$, $\pr$ and is reported by $\op{a}$ to have read the value associate to timestamp $ts$.

\renewcommand{\toto}{lemma:async:unbound:Completeness}
\end{proofL}

\begin{lemma}
\label{lemma:async:unbound:CompletenessCollusion}
Algorithm presented figure \ref{alg:async:unbound:AtomicRegisterClientWrite} to \ref{alg:async:unbound:AtomicRegisterServer} 
% with $\tau \geq 2f+1$ and $t \leq \tau-2f$ 
solves the completeness (with collusion) property
\end{lemma}\spaceLemmaProof 
\begin{proofL}
 For a reader $\pr$ to returns for a valid value $v$ with timestamp $ts$, then $\pr$ receives at least $\tau$ messages from different servers (line \ref{line:async:unbound:conditionread} figure \ref{alg:async:unbound:AtomicRegisterClientRead}) with the block corresponding to $v$. Notice that if $\pr$ is faulty, it can also receive those blocks not directly from the servers but for some other faulty process in $\FaultySet$. However, those other faulty process at some point must have receives those blocks from the servers.
 
 A correct server sends a block with associate timestamp $ts$ to a reader $\pr'$ (line \ref{line:async:unbound:sendVal}, figure \ref{alg:async:unbound:AtomicRegisterServer}), only after it adds to its log the reader $\pr'$ associate with timestamp $ts$ (line \ref{line:async:unbound:logServRval} figure \ref{alg:async:unbound:AtomicRegisterServer}). Thus, if a correct server $\pss$ sends a block with associate timestamp $ts$ to a reader $\pr'$, $\pss$ stores $\pr'$ ID associate with $ts$ in its log. If $\tau\geq 2f+1$, since there is at most $f$ Byzantine, in the worst case, at least $\tau-f\geq f+1$ correct servers, denoted $P_C$, records in their logs directly the reader $\pr$, or if $\pr$ is faulty, some faulty process in $\FaultySet$.

Let $\op{a}$ be an audit operation, invoked by a process $\pa$, that starts after $\pr$ returns.
So when $\op{a}$ starts, $\pr$ is in PC's log. Then, $\pa$ waits $2f+1$ responses (line \ref{line:async:unbound:waitAuditResponse} figure \ref{alg:async:unbound:AtomicRegisterClientWrite}) after sending $\AUDIT$ request (line \ref{line:async:unbound:auditRequest} figure \ref{alg:async:unbound:AtomicRegisterClientWrite}) to servers. As there is at most $f$ Byzantine servers, $\pa$ gets the responses from at least $f+1$ ($n-2f$) correct servers. In particular, $\pa$ get at least one response from a server in $P_C$. Finally, with $t\leq\tau-2f=1$, if $\pr$ is correct, $\pr$ is reported by $\op{a}$ to have read the value associate to timestamp $ts$, otherwise some faulty process in $\FaultySet$ are.

\renewcommand{\toto}{lemma:async:unbound:CompletenessCollusion}
\end{proofL}

\begin{lemma}
\label{lemma:async:unbound:StrongAccuraySignedMessage}
Algorithm presented figure \ref{alg:async:unbound:AtomicRegisterClientWrite} to \ref{alg:async:unbound:AtomicRegisterServer} with $t \geq 1$ solves the strong accuracy property
\end{lemma}\spaceLemmaProof 

\begin{proofL}
We have to prove that a correct reader $\pr$ that never invoked a read operation cannot be reported by an audit operation. With $t=1$, a reader $\pr$ is reported by an audit operation if one server respond to the $\AUDIT$ message with a correct record of $\pr$ in its log. Thanks to the use of signature, a false record cannot be created by a Byzantine server. The signature used to attest the validity of a record are of two kind. If a correct server add $\pr$ in its log before responding to $\GetValUnbound$ messages (line \ref{line:async:unbound:logServRval}, figure \ref{alg:async:unbound:AtomicRegisterServer}), then it uses the reader signature. So for a process to have a valid record to $\pr$ in its log, the process $\pr$ must have sent $\GetValUnbound$ messages to some servers,  i.e. $\pr$ must have invoked a read operation.

\renewcommand{\toto}{lemma:async:unbound:StrongAccuraySignedMessage}

\end{proofL}

\begin{theorem}
\label{theorem:async:unbound:StrongauditabilitySignedMessage}
Algorithm presented figure \ref{alg:async:unbound:AtomicRegisterClientWrite} to \ref{alg:async:unbound:AtomicRegisterServer} with $n=3f+1$, $\tau = 2f+1$ and $t=1$ solves the strong auditability property
\end{theorem}

\begin{proofT}
Directly from Lemma \ref{lemma:async:unbound:StrongAccuraySignedMessage} and Lemma \ref{lemma:async:unbound:Completeness} with $t=1$ and $\tau=2f+1$.


\renewcommand{\toto}{theorem:async:unbound:StrongauditabilitySignedMessage}
\end{proofT}


==> proof/livenessUnbound.tex <==


\begin{lemma}
\label{lemma:async:unbound:writeliveness}
If $\pw$ is correct (if the writer don't crash), then each write operation invoked by $\pw$ eventually terminates.
\end{lemma}\spaceLemmaProof 


\begin{proofL}
The write operation has the following structure. The writer broadcasts a  $\writets$ message to all servers (line \ref{line:async:unbound:writeTs} of Figure \ref{alg:async:unbound:AtomicRegisterClientWrite}) and waits $n-f$ ACKs (line \ref{line:async:unbound:writeTsWaitAck} of Figure \ref{alg:async:unbound:AtomicRegisterClientWrite}) from different servers before terminate.

Since $\pw$ is correct, the channel communications properties assure that all correct servers deliver the message $\writets$ broadcast by $\pw$. Considering that: (i) servers do not apply any condition to send back $\writetsack$ messages (line \ref{line:async:unbound:writeAck} of Figure \ref{alg:async:unbound:AtomicRegisterServer}), and that (ii) at most $f$ servers can be faulty, $\pw$ always receives the $n-f$ $\writetsack$ replies from correct servers necessary to stop waiting, which concludes the proof.

\renewcommand{\toto}{lemma:async:unbound:writeliveness}
\end{proofL}


\begin{lemma}
\label{lemma:async:unbound:WriteRtsUpdate}
Let $\op{w}$ be a complete write operation that writes $v$ with timestamp $ts$. If a correct server $\pss$ updates $\Rts$ with $ts$, then all correct servers eventually adds the block corresponding to $v$ in  $\RVal$.

\end{lemma}\spaceLemmaProof  

\begin{proofL}
Let us recall that a correct server updates $\Rts$ with $ts$ only upon receiving a $\writets$ message (line \ref{line:async:unbound:receiveWriteVal} figure \ref{alg:async:unbound:AtomicRegisterServer}).
When a server updates $\Rts$ with $ts$, it also add to $\RVal$ (line \ref{line:async:unbound:updateRValWriteVal} figure \ref{alg:async:unbound:AtomicRegisterServer}) the associate block it receives in the $\writets$ message from the writer (line \ref{line:async:unbound:receiveWriteVal} figure \ref{alg:async:unbound:AtomicRegisterServer}). As there is a reliable broadcast between the writer and servers, eventually all correct servers receive the $\writets$ message and updates $\RVal$ with their block associate to $ts$.
% with the value it stores in $\RNextVal$. As the writer is correct and due to the FIFO order of the channel of communication between the writer and the servers, if a server updates $\Rts$ with timestamp $ts$, then the value it stores in $\RNextVal$ is associate with timestamp $ts$. Finally, as there is a reliable broadcast between the writer and the servers, all correct server eventually receive $\writets$ message and update $\RVal$ with value associate to ts.

\renewcommand{\toto}{lemma:async:unbound:WriteRtsUpdate}
\end{proofL}

\begin{lemma}
\label{lemma:async:unbound:smallestTimestampRts}
When a correct reader $\pr$ receives the response to $\getts$ from all correct servers, in at least one correct server $\Rts\geq\smallestTimestamp$.
\end{lemma}\spaceLemmaProof 

\begin{proofL}
By contradiction, assume that in all correct servers $\Rts<\smallestTimestamp$. 

Then, in response to $\getts$ messages, all correct servers send their $\Rts$, all inferior to $\smallestTimestamp$. We note $tsMax$ the greatest timestamp receives by $\pr$ from correct servers. Then, it exists in $\collectedTs$ $2f+1$ timestamp $\leq tsMax$. By assumption, $tsMax<\smallestTimestamp$, which is in contradiction with the condition line \ref{line:async:unbound:notOld}.

\renewcommand{\toto}{lemma:async:unbound:smallestTimestampRts}
\end{proofL}

% \begin{figure}[!ht]
% \centering
%     \includegraphics[scale=0.252]{image/scenario/Scenario_t_gotts.PNG}
%     \caption{Scenario $\gtso$}
%     \label{fig:scenario:unbound:gotts}
% \end{figure}

\begin{lemma}
\label{lemma:async:unbound:ReadTermination}
A read operation $\op{r}$ invoked by a correct process $\pr$ always terminates.
\end{lemma}\spaceLemmaProof  

\begin{proofL}
First, observe that if $\pr$ satisfies the conditions at line \ref{line:async:unbound:conditionread} figure \ref{alg:async:unbound:AtomicRegisterClientRead}, $\pr$ terminates.
Then, let us show by construction that those conditions are necessarily satisfied. 

A correct reader $\pr$ starts the read operation, after it reinitialized all the variables. Then, $\pr$ sends a $\getts$ messages to all the servers. Consider the moment $\pr$ receives the response from the $2f+1$ correct servers, and sends a $\GetValUnbound$ message to all the servers for timestamp $\smallestTimestamp$. Notice that according to Lemma \ref{lemma:async:unbound:smallestTimestampRts} at least one correct server has set $\Rts$ to $\smallestTimestamp$. As at least one correct server set $\Rts$ to $\smallestTimestamp$, then from the reliable broadcast, eventually all servers will set $\Rts$ to $\smallestTimestamp$. Then, the reader will eventually receive the $2f+1$ response from correct servers such that the condition line \ref{line:async:unbound:conditionGetBlock} is satisfied. 

Then the reader sends $\GetBlocks$ messages for timestamp $\smallestTimestamp$ to all servers. As at least one correct server set $\Rts$ to $\smallestTimestamp$, from Lemma \ref{lemma:async:unbound:WriteRtsUpdate}, eventually all correct servers have in $\RVal$ the block associate with timestamp $\smallestTimestamp$. Then, in response to $\GetBlocks$, all correct servers can send their block corresponding to timestamp $ts$ and the condition $\ValidBlock$ is satisfied, such that the reader can return for the value-timestamp pair corresponding to timestamp $ts$.

\renewcommand{\toto}{lemma:async:unbound:ReadTermination}
\end{proofL}


==> proof/verystrong/atomicity.tex <==


According to line \ref{line:async:unboundStrong:updateRts} figure \ref{alg:async:unboundStrong:AtomicRegisterServer}
% \ref{line:async:unboundStrong:writetsRts} figure \ref{alg:async:unboundStrong:AtomicRegisterServer}
the following observation holds :

\begin{observation}
\label{observation:unbound:tsMonotonicallyIncrease}
A correct server $\ps{i}$ updates $\Rts$ with a new timestamp, only if this timestamp is greater than the previous one stored in $\Rts$. Hence, timestamps stored at correct servers increase monotonically
\end{observation}

\noindent{}
\begin{lemma}
\label{lemma:async:unboundStrong:writerEndWriteServerTimestamp}
Let $\op{w}$ be a write operation with timestamp $ts$. After $\op{w}$ returns the value of $\Rts$ is greater than or equal to $ts$ in at least $f+1$ correct servers. 

\end{lemma}\spaceLemmaProof 

\begin{proofL}
$\op{w}$ terminates when the condition at line \ref{line:async:unboundStrong:writeTsWaitAck} of figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite} is evaluated to true. 
Hence, $\op{w}$ terminates only if the writer received  $(\writetsack,ts)$, from at least $2f+1$ different servers. 
A correct server, sends $(\writetsack,ts)$ (line \ref{line:async:unboundStrong:writeAck} of figure \ref{alg:async:unboundStrong:AtomicRegisterServer}) to the writer, if it receives $(\writets,ts,-,-,-)$ from the writer and after the execution of line \ref{line:async:unboundStrong:updateRts} in Figure \ref{alg:async:unboundStrong:AtomicRegisterServer}
Since there are at most $f$ of the $3f+1$ servers are Byzantine, once the write operation completes, the writer has received at least $f+1$  $(\writetsack,ts)$ from correct servers.
Observation \ref{observation:unbound:tsMonotonicallyIncrease} concludes the proof. 

\renewcommand{\toto}{lemma:async:unboundStrong:writerEndWriteServerTimestamp}
\end{proofL}



\begin{lemma}
\label{lemma:async:unboundStrong:readerEndWriteServerTimestamp}
Let $\op{r}$ be a complete read operation and let $ts$ the timestamp corresponding to the value it returns. At any time after $\op{r}$ returns the value of $\Rts$ is greater than or equal to $ts$ in at least $f+1$ correct servers. 
\end{lemma}\spaceLemmaProof 


\begin{proofL}
Since $\op{r}$ terminates, it has satisfied the condition $\ValidBlock(ts)$ (line \ref{line:async:unboundStrong:conditionread} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}). For this condition to be true, the reader must have received $2f+1$ different valid blocks for timestamp $ts$, piggybacked by $\VALS$ messages (lines \ref{line:async:unboundStrong:valRepColectTs} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) sent by different servers. A correct server sends such messages, only after it has $\Rts\geq ts$ (lines \ref{line:async:unboundStrong:waitTsSendVal} and \ref{line:async:unboundStrong:updateRts}).
Since there are at most $f$ Byzantine servers, and by observation \ref{observation:unbound:tsMonotonicallyIncrease}, the claims follow.

\renewcommand{\toto}{lemma:async:unboundStrong:readerEndWriteServerTimestamp}
\end{proofL}


\begin{lemma}
\label{lemma:async:unboundStrong:W-Ratomicity}
Let $\op{w}$ be a complete write operation with timestamp $ts$ and let $\op{r}$ be a complete read operation by a correct process $\pr$ associated to a timestamp $ts'$. If $\op{r}$ succeeds $\op{w}$ in real-time order then $ts' \geq ts$
\end{lemma}\spaceLemmaProof 

\begin{proofL}
Since $\op{r}$ returns a value associated to timestamp $ts'$, the condition $\notOld(ts')$ (line \ref{line:async:unboundStrong:conditionread} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) is satisfied. 
In the following, we show that $\notOld(ts')$ true implies that $ts'\geq ts$.

Let us consider that $\notOld(ts')$ is true. 
As $\collectedTs$ is reinitialized at the beginning of each new read operation, $\notOld(ts')$ is true, if all timestamps receives from at least $2f+1$ different servers piggybacked by $\SendValUnbound$ (line \ref{line:async:unboundStrong:valRepColectTs} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) or $\TS$ (line \ref{line:async:unboundStrong:valRepColectTs} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) messages are smaller than or equal to $ts'$.
According to Lemma \ref{lemma:async:unboundStrong:writerEndWriteServerTimestamp}, as $\op{w}$ terminates, the content of $\Rts$ is greater than or to equal  $ts$ in at least $f+1$ correct servers.
So, during $\op{r}$, in response to $(\getval,\nSeq)$ (line \ref{line:async:unboundStrong:sendVal} figure \ref{alg:async:unboundStrong:AtomicRegisterServer}), the reader can collect at most $2f=n-(n-2f)$ messages for a timestamp smaller than $ts$. Thus, $\notOld()$ always remain false for any timestamp smaller than $ts$, and since $\notOld(ts')$ is true,  $ts'\geq ts$.



\renewcommand{\toto}{lemma:async:unboundStrong:W-Ratomicity}

\end{proofL}

\begin{lemma}
\label{lemma:async:unboundStrong:returnWrittenValue}
If a complete read operation $\op{r}$, invoked by a correct process $\pr$,  returns a value corresponding to a timestamp $ts>0$, then it exists a write operation $\op{w}$, with timestamp $ts$, that starts before $\op{r}$ terminates.

\end{lemma}\spaceLemmaProof 
\begin{proofL}
Since $\op{r}$ terminates, it has satisfied the condition $\ValidBlock(ts)$ (line \ref{line:async:unboundStrong:conditionread} of Figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}). Thus, the reader received $2f+1$ distinct valid blocks for timestamp $ts$, piggybacked by $\SendBlock$  messages (lines \ref{line:async:unboundStrong:receiveGetBlocks} and of Figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) sent by distinct servers. As all the variables are reinitialized at the beginning of a read operation, and as there are at most $f$ Byzantine servers, at least $f+1$  correct servers sent a block to $\pr$ during the execution of $\op{r}$. 
A correct server $\pss$ sends a block corresponding to a timestamp $ts>0$ only after it has received the corresponding $\writets$ message from the writer; thus, after the invocation of a write operation $\op{w}$ for timestamp $ts$. It follows that $\op{w}$ began before $\op{r}$ completes.

\renewcommand{\toto}{lemma:async:returnWrittenValue}
\end{proofL}


\begin{lemma} 
\label{lemma:async:unboundStrong:R-Ratomicity}
Let $\op{r}$ be a complete read operation invoked by a correct process $\pr$, and let $\op{r'}$ be a complete read operation invoked by a correct process $\pr'$ ($\pr$ and $\pr'$ may be the same process). Let $ts$ and $ts'$ be the timestamps associated with $\op{r}$ and $\op{r'}$ respectively. If $\op{r'}$ succeeds $\op{r}$  in real-time order then $ts' \geq ts$.

\end{lemma}\spaceLemmaProof 

\begin{proofL}
The proof follows the same approach as the proof of Lemma \ref{lemma:async:unboundStrong:W-Ratomicity}.

Let $ts'$ be $\op{r'}.ts$ and let $ts$ be $\op{r}.ts$.
As $\op{r'}$ returns a value associated to a timestamp $ts'$, the conditions $\ValidBlock(ts')$ and $\notOld(ts')$ are true for timestamp $ts$ (line \ref{line:async:unboundStrong:conditionread} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}). 
In the following, we show that if condition $\notOld(ts')$ implies that $ts'\geq ts$.

Let us consider that $\notOld(ts')$ is true. 
As $\collectedTs$ is reinitialized at the beginning of each new read operation, $\notOld(ts')$ is true, if all timestamps receives from at least $2f+1$ different servers piggybacked by $\SendValUnbound$ (line \ref{line:async:unboundStrong:valRepColectTs} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) or $\TS$ (line \ref{line:async:unboundStrong:valRepColectTs} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) messages are smaller than or equal to $ts'$.
According to Lemma \ref{lemma:async:unboundStrong:readerEndWriteServerTimestamp}, as $\op{r}$ returns for timestamp $ts$, then at server side, the content of $\Rts$ is greater than or to equal  $ts$ in at least $f+1$ correct servers.
So the reader can collect at most $2f=n-(n-2f)$  timestamps smaller than $ts$. Thus, $\notOld$ always remain false for any timestamp smaller than $ts$, hence $ts'\geq ts$.

\renewcommand{\toto}{lemma:async:unboundStrong:R-Ratomicity}
\end{proofL}

\begin{lemma} 
\label{lemma:async:unboundStrong:R-Watomicity}
Let $\op{r}$ be a complete read operation with timestamp $ts$ and let $\op{w}$ be a complete write operation by $\pw$ associated to a timestamp $ts'$. 
If $\op{w}$ succeeds $\op{r}$ in real-time order then $ts' \geq ts$
\end{lemma}\spaceLemmaProof 

\begin{proofL}
We proceed considering first the case in which $ts>0$ and then the case in which $ts=0$.
From Lemma \ref{lemma:async:unboundStrong:returnWrittenValue}, if $ts>0$ then it exists $\op{w'}$ with timestamp $ts$ that starts before the end of $\op{r}$. Considering that, there is a unique writer and that its execution is sequential, then $\op{w'}$ terminates before $\op{w}$ starts. As timestamps growth monotonically (Observation \ref{observation:unbound:tsMonotonicallyIncrease}), 
$ts'>ts$.

Consider now the case $ts=0$. As timestamps grow monotonically (Observation \ref{observation:unbound:tsMonotonicallyIncrease}), and the initial value of the timestamp is $0$ (line \ref{line:async:unboundStrong:initTs} of Figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite}) then all write operations have their timestamp greater than $0$. In particular this is true for $\op{w}$, such that $ts'>ts$, which concludes the proof.
\renewcommand{\toto}{lemma:async:unboundStrong:R-Watomicity}
\end{proofL}


% \begin{lemma}
% \label{lemma:async:unboundStrong:Safety}
% If a read operation $\op{r}$, invoked by a correct process $\pr$ and not concurrent to any write operation, returns a value $v$, then $v$ is the value of the most recently preceding write. If there is none, $v$ is the initial value $\vo$.

% \end{lemma}\spaceLemmaProof 

% \begin{proofL}
% First we consider the cases where there is no preceding write operation, and then the case where there is one.

% Let us show by contradiction that, when there is no preceding write operation to $\op{r}$, it is impossible that $\op{r}$ returns for $v'\neq \vo$.
% In this case, as there is no write operation corresponding to $v'$, it is impossible for correct servers to send a message with a block corresponding to $v'$. However, for $\pr$  to read $v'$, the condition $\ValidBlock(ts')$ (line \ref{line:async:unboundStrong:conditionread} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) must be satisfied. Thus, $\pr$ must  collect $2f+1$ blocks for $ts'$ from different servers in $\SendBlock$ messages. By the property of none creation of the canal of communication, $\pr$ cannot receive such messages from correct servers.Thus, $\pr$ receives those blocks from $2f+1$ Byzantine servers. As there are at most $f$ Byzantine, this is a contradiction. 

% Now, we consider the cases where a preceding write operation exists, $\op{w}$, that writes $v$ with associate timestamp $ts$. Let us show that $\op{r}$ cannot return a value $v'\neq v$. Notice that values are identifiable with their timestamp, such that $v'\neq v \Longleftrightarrow ts'\neq ts$, with $ts'$ the timestamp associate with $v'$. There are two cases to consider, (i) $ts'>ts$ and (ii) $ts'<ts$.  In case (i), $ts'>ts$, as by assumption the last write operation is $\op{w}$, and that timestamp grows monotonically (Observation \ref{observation:unbound:tsMonotonicallyIncrease}), there is no write operation  corresponding to $ts'$. Then the same arguments as before apply and gives the contradiction. In case (ii), $ts'<ts$, Lemma \ref{lemma:async:unboundStrong:W-Ratomicity} gives the contradiction and concludes the proof.

% \renewcommand{\toto}{lemma:async:unboundStrong:Safety}
% \end{proofL}


% \begin{theorem}
% \label{theorem:async:unboundStrong:linearizable}
% There is a permutation $\pi$ of all completed operations in $\eventSeq$ and some subset of the pending operations such that
% if the response of operation $\op{1}$ occurs in $\eventSeq$, before the invocation of operation $\op{2}$, then $\op{1}$ appears before $\op{2}$ in $\pi$
% \end{theorem}

% \begin{proofT}
% We consider a sequence of event $\eventSeq$. In the following, we describe how to create such a permutation $\pi$ of operation. First, for each incomplete write operation $\op{w}\in\eventSeq$ associate with a value $v$, if it exists a read operation $\op{r}\in\eventSeq$ that returns $v$, then we complete $\op{w}$.

% Then, we order the operations according to their timestamp. For write operation and a read operation with the same timestamp, we order write operation before reads, and we order read operation with the same timestamp according to real time execution. Thus, from Lemma \ref{lemma:async:unboundStrong:W-Ratomicity} and Lemma \ref{lemma:async:unboundStrong:R-Ratomicity} if the response of an operation $\op{1}$ occurs before the invocation of an operation $\op{2}$, then $\op{1}$ appears before $\op{2}$ in $\pi$.

% \renewcommand{\toto}{theorem:async:unboundStrong:linearizable}
% \end{proofT}





Let $E$ be any execution of our algorithm and let $H$ be the corresponding history. 
We construct ${\sf complete}(H)$ by removing all the invocations of the read operations that have no matching response and by completing a pending $write(v)$ operation if there is a complete read operation that returns $v$. Observe that only the last write operation of the writer can be pending.

Then, we explicitly construct a sequential history $\pi$ containing all the operations in ${\sf complete}(H)$. 
First we put in $\pi$ all the write operations according to the order in which they occur in $H$, because write operations are executed sequentially by the unique writer, this sequence is well-defined. Also this order is consistent with that of the timestamps associated with the values written.

Next, we add the read operations one by one, in the order of their response in $H$. A read operation that returns a value with timestamp $ts$ is placed immediately before the write that follows in $\pi$ the write operation associated to $ts$ (or at the end if this write does not exist). By construction of $\pi$ every read operation returns the value of the last preceding write in $\pi$. 
It remains to prove that $\pi$ preservers the real-time order of non-overlapping operations.
\\
\begin{theorem} \label{theorem:async:unboundStrong:linearizable}
Let $\op{1}$ and $\op{2}$ be two operations in $H$. If $\op{1}$ ends before the invocation of $\op{2}$ then $\op{1}$ precedes $\op{2}$ in $\pi$.

\end{theorem}\spaceLemmaProof

\begin{proofT}

Since $\pi$ is consistent with the order of timestamps, we have to show that the claim is true for all operations with different timestamps.

There are four possible scenarios: 
$\op{1}$ and $\op{2}$ are respectively a write and a read operation, then the claim holds by Lemma \ref{lemma:async:unboundStrong:W-Ratomicity}.
$\op{1}$ and $\op{2}$ are two reads operations, then the claim holds by Lemma \ref{lemma:async:unboundStrong:R-Ratomicity}. 
$\op{1}$ and $\op{2}$ are respectively a read and a write operation, then the claim holds by Lemma \ref{lemma:async:unboundStrong:R-Watomicity}.
If $\op{1}$ and $\op{2}$ are two write operations the claim holds by the Observation \ref{observation:unbound:tsMonotonicallyIncrease}.

\renewcommand{\toto}{theorem:async:linearizable}
\end{proofT}



==> proof/verystrong/auditability.tex <==

\begin{lemma}
\label{lemma:async:unboundStrong:Completeness}
Algorithm presented figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite} to \ref{alg:async:unboundStrong:AtomicRegisterServer} 
% with $\tau \geq 2f+1$ and $t \leq \tau-2f$ 
solves the completeness property
\end{lemma}\spaceLemmaProof 
\begin{proofL}
 For a reader $\pr$ to returns for a valid value $v$ with timestamp $ts$, then $\pr$ receives at least $\tau$ messages from different servers (line \ref{line:async:unboundStrong:conditionread} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}) with the block corresponding to $v$.
 A correct server sends a block corresponding to value associate with timestamp $ts$ to a reader $\pr$ (line \ref{line:async:unboundStrong:sendVal}, figure \ref{alg:async:unboundStrong:AtomicRegisterServer}), only after it adds to its log the reader $\pr$ associate with timestamp $ts$, line \ref{line:async:unboundStrong:logServRval} figure \ref{alg:async:unboundStrong:AtomicRegisterServer}. Thus, if a correct server $\pss$ sends a block with associate timestamp $ts$ to a reader $\pr$, $\pss$ stores $\pr$ ID associate with $ts$ in its log. If $\tau\geq 2f+1$, since there is at most $f$ Byzantine, in the worst case, at least $\tau-f\geq f+1$ correct servers, denoted $P_C$, records $\op{r}$ in their logs. 

Let $\op{a}$ be an audit operation, invoked by a process $\pa$, that starts after $\pr$ returns.
So when $\op{a}$ starts, $\pr$ is in PC's log. Then, $\pa$ waits $2f+1$ responses (line \ref{line:async:unboundStrong:waitAuditResponse} figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite}) after sending $\AUDIT$ request (line \ref{line:async:unboundStrong:auditRequest} figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite}) to servers. As there is at most $f$ Byzantine servers, $\pa$ gets the responses from at least $f+1$ ($n-2f$) correct servers. In particular, $\pa$ get at least one response from a server in $P_C$. Finally, with $t\leq\tau-2f=1$, $\pr$ and is reported by $\op{a}$ to have read the value associate to timestamp $ts$.

\renewcommand{\toto}{lemma:async:unboundStrong:Completeness}
\end{proofL}

\begin{lemma}
\label{lemma:async:unboundStrong:StrongAccuraySignedMessage}
Algorithm presented figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite} to \ref{alg:async:unboundStrong:AtomicRegisterServer} with $t \geq 1$ solves the strong accuracy property
\end{lemma}\spaceLemmaProof 

\begin{proofL}
We have to prove that a correct reader $\pr$ that never invoked a read operation cannot be reported by an audit operation. With $t=1$, a reader $\pr$ is reported by an audit operation if one server respond to the $\AUDIT$ message with a correct record of $\pr$ in its log. Thanks to the use of signature, a false record cannot be created by a Byzantine server. The signature used to attest the validity of a record are of two kind. If a correct server add $\pr$ in its log before responding to $\GetValUnbound$ messages (line \ref{line:async:unboundStrong:logServRval}, figure \ref{alg:async:unboundStrong:AtomicRegisterServer}), then it uses the reader signature. So for a process to have a valid record to $\pr$ in its log, the process $\pr$ must have sent $\GetValUnbound$ messages to some servers,  i.e. $\pr$ must have invoked a read operation.

\renewcommand{\toto}{lemma:async:unboundStrong:StrongAccuraySignedMessage}

\end{proofL}

\begin{theorem}
\label{theorem:async:unboundStrong:StrongauditabilitySignedMessage}
Algorithm presented figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite} to \ref{alg:async:unboundStrong:AtomicRegisterServer} with $n=3f+1$, $\tau = 2f+1$ and $t=1$ solves the strong auditability property
\end{theorem}

\begin{proofT}
Directly from Lemma \ref{lemma:async:unboundStrong:StrongAccuraySignedMessage} and Lemma \ref{lemma:async:unboundStrong:Completeness} with $t=1$ and $\tau=2f+1$.


\renewcommand{\toto}{theorem:async:unboundStrong:StrongauditabilitySignedMessage}
\end{proofT}


==> proof/verystrong/liveness.tex <==


\begin{lemma}
\label{lemma:async:unboundStrong:writeliveness}
If $\pw$ is correct (if the writer don't crash), then each write operation invoked by $\pw$ eventually terminates.
\end{lemma}\spaceLemmaProof 


\begin{proofL}
The write operation has the following structure. The writer broadcasts a  $\writets$ message to all servers (line \ref{line:async:unboundStrong:writeTs} of Figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite}) and waits $n-f$ ACKs (line \ref{line:async:unboundStrong:writeTsWaitAck} of Figure \ref{alg:async:unboundStrong:AtomicRegisterClientWrite}) from different servers before terminate.

Since $\pw$ is correct, the channel communications properties assure that all correct servers deliver the message $\writets$ broadcast by $\pw$. Considering that: (i) servers do not apply any condition to send back $\writetsack$ messages (line \ref{line:async:unboundStrong:writeAck} of Figure \ref{alg:async:unboundStrong:AtomicRegisterServer}), and that (ii) at most $f$ servers can be faulty, $\pw$ always receives the $n-f$ $\writetsack$ replies from correct servers necessary to stop waiting, which concludes the proof.

\renewcommand{\toto}{lemma:async:unboundStrong:writeliveness}
\end{proofL}


\begin{lemma}
\label{lemma:async:unboundStrong:WriteRtsUpdate}
Let $\op{w}$ be a complete write operation that writes $v$ with timestamp $ts$. If a correct server $\pss$ updates $\Rts$ with $ts$, then all correct servers eventually adds the block corresponding to $v$ in  $\RVal$.

\end{lemma}\spaceLemmaProof  

\begin{proofL}
Let us recall that a correct server updates $\Rts$ with $ts$ only upon receiving a $\writets$ message (line \ref{line:async:unboundStrong:receiveWriteVal} figure \ref{alg:async:unboundStrong:AtomicRegisterServer}).
When a server updates $\Rts$ with $ts$, it also add to $\RVal$ (line \ref{line:async:unboundStrong:updateRValWriteVal} figure \ref{alg:async:unboundStrong:AtomicRegisterServer}) the associate block it receives in the $\writets$ message from the writer (line \ref{line:async:unboundStrong:receiveWriteVal} figure \ref{alg:async:unboundStrong:AtomicRegisterServer}). As there is a reliable broadcast between the writer and servers, eventually all correct servers receive the $\writets$ message and updates $\RVal$ with their block associate to $ts$.
% with the value it stores in $\RNextVal$. As the writer is correct and due to the FIFO order of the channel of communication between the writer and the servers, if a server updates $\Rts$ with timestamp $ts$, then the value it stores in $\RNextVal$ is associate with timestamp $ts$. Finally, as there is a reliable broadcast between the writer and the servers, all correct server eventually receive $\writets$ message and update $\RVal$ with value associate to ts.

\renewcommand{\toto}{lemma:async:unboundStrong:WriteRtsUpdate}
\end{proofL}

\begin{lemma}
\label{lemma:async:unboundStrong:smallestTimestampRts}
When a correct reader $\pr$ receives the response to $\getts$ from all correct servers, in at least one correct server $\Rts\geq\smallestTimestamp$.
\end{lemma}\spaceLemmaProof 

\begin{proofL}
By contradiction, assume that in all correct servers $\Rts<\smallestTimestamp$. 

Then, in response to $\getts$ messages, all correct servers send their $\Rts$, all inferior to $\smallestTimestamp$. We note $tsMax$ the greatest timestamp receives by $\pr$ from correct servers. Then, it exists in $\collectedTs$ $2f+1$ timestamp $\leq tsMax$. By assumption, $tsMax<\smallestTimestamp$, which is in contradiction with the condition line \ref{line:async:unboundStrong:notOld}.

\renewcommand{\toto}{lemma:async:unboundStrong:smallestTimestampRts}
\end{proofL}

% \begin{figure}[!ht]
% \centering
%     \includegraphics[scale=0.252]{image/scenario/Scenario_t_gotts.PNG}
%     \caption{Scenario $\gtso$}
%     \label{fig:scenario:unbound:gotts}
% \end{figure}

\begin{lemma}
\label{lemma:async:unboundStrong:ReadTermination}
A read operation $\op{r}$ invoked by a correct process $\pr$ always terminates.
\end{lemma}\spaceLemmaProof  

\begin{proofL}
First, observe that if $\pr$ satisfies the conditions at line \ref{line:async:unboundStrong:conditionread} figure \ref{alg:async:unboundStrong:AtomicRegisterClientRead}, $\pr$ terminates.
Then, let us show by construction that those conditions are necessarily satisfied. 

A correct reader $\pr$ starts the read operation, after it reinitialized all the variables. Then, $\pr$ sends a $\getts$ messages to all the servers. Consider the moment $\pr$ receives the response from the $2f+1$ correct servers, and sends a $\GetValUnbound$ message to all the servers for timestamp $\smallestTimestamp$. Notice that according to Lemma \ref{lemma:async:unboundStrong:smallestTimestampRts} at least one correct server has set $\Rts$ to $\smallestTimestamp$. As at least one correct server set $\Rts$ to $\smallestTimestamp$, then from the reliable broadcast, eventually all servers will set $\Rts$ to $\smallestTimestamp$. Then, the reader will eventually receive the $2f+1$ response from correct servers such that the condition line \ref{line:async:unboundStrong:conditionGetBlock} is satisfied. 

Then the reader sends $\GetBlocks$ messages for timestamp $\smallestTimestamp$ to all servers. As at least one correct server set $\Rts$ to $\smallestTimestamp$, from Lemma \ref{lemma:async:unboundStrong:WriteRtsUpdate}, eventually all correct servers have in $\RVal$ the block associate with timestamp $\smallestTimestamp$. Then, in response to $\GetBlocks$, all correct servers can send their block corresponding to timestamp $ts$ and the condition $\ValidBlock$ is satisfied, such that the reader can return for the value-timestamp pair corresponding to timestamp $ts$.

\renewcommand{\toto}{lemma:async:unboundStrong:ReadTermination}
\end{proofL}


==> relatedWork.tex <==
% Many systems provide different level of consistency in a total untrusted server environment,  making different fault assumption for the client. Most of them are based on a hash chain system, SUNDR \cite{sundr04} provide fork consistency with malicious client, Venus \cite{venus10} provide eventual consistency with correct client, Caelus \cite{caelus15} provide eventual consistency but does not resist collusion of the server and the client, SPORC \cite{sporc10} combines fork consistency and operational transformation with correct client, Depot \cite{depot11} provide Fork-Join-Casual consistency with malicious client, CloudProof \cite{cloudproof10} provide write-serializability with malicious client, Ghostor \cite{ghostor20} provide Verifiable Linearisability with malicious client. IRIS \cite{iris12} also provide retrievability thanks to a dynamic PoR. Other system provide consistency in presence of  $f$ replicas Byzantine, this is the case of DepSky\cite{depsky}. DepSky use a cloud of cloud approach using several cloud providers to implement a solution using Byzantine quorum system protocols\cite{malkhi98}, which guarantee consistency in presence of faulty readers and crash for writers. Other protocol provide atomic semantic in presence of entirely Byzantine clients\cite{cachin_optimal06}\cite{cachin_asynchronous05} by using server specific protocols and Information Dispersal\cite{rabin_efficient89}.

% \todo{paragraph to explain the differences with respect to Bessani. Their results and conjectures. We proved their conjecture (f replicas more for auditability) and extended their results with a protocol 3f+1 with server to server comm. To see if it would be better to have a list}


